Intrinsically Reliable and Lightweight Physical Obfuscated Keys

Physical Obfuscated Keys (POKs) allow tamper-resistant storage of random keys based on physical disorder. The output bits of current POK designs need to be first corrected due to measurement noise and next de-correlated since the original output bits may not be i.i.d. (independent and identically distributed) and also public helper information for error correction necessarily correlates the corrected output bits.For this reason, current designs include an interface for error correction and/or output reinforcement, and privacy amplification for compressing the corrected output to a uniform random bit string. We propose two intrinsically reliable POK designs with only XOR circuitry for privacy amplification (without need for reliability enhancement) by exploiting variability of lithographic process and variability of granularity in phase change memory (PCM) materials. The two designs are demonstrated through experiments and simulations.

==> Draft_eprint - Copy/sections/abstract.tex <==
\begin{abstract}
Physical Obfuscated Keys (POKs) allow tamper-resistant storage of random keys based on physical disorder. 
The output bits of current POK designs need to be first corrected due to measurement noise and next de-correlated since the original output bits may not be i.i.d. (independent and identically distributed) and also public helper information for error correction necessarily correlates the corrected output bits.
%The output of current POK designs need to be corrected and de-correlated due to measurement noise and the correlation in hardware. 
For this reason, current designs include an interface for error correction and/or output reinforcement, and privacy amplification for compressing the corrected output to a uniform random bit string. We propose two intrinsically reliable POK designs with only XOR circuitry for privacy amplification (without need for reliability enhancement) by exploiting \textbf{variability of lithographic process and variability of granularity in phase change memory (PCM) materials}. The two designs are demonstrated through experiments and simulations. 
\end{abstract}

%\category{SEC1.4}{Emerging technologies and security (Nano, 3D, FPGA, etc.)}{}[]


%\terms{Security, Design, Phase Change Memory, Lithography, Physical Obfuscated Key, Physical Unclonable Function}

==> Draft_eprint - Copy/sections/acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:Acknowledgements}
The devices are fabricated at IBM T.J. Watson Research Center
and characterized at UConn, supported by the U. S. National
Science Foundation under awards \# ECCS 0925973 and ECCS
1150960. The characterization and analysis efforts of R.S.K., N.N. and J.S. and the problem statement and motivation of C.J. and H.P.N. are supported by 
%Multidisciplinary University Research Initiatives (MURI) Program. 
%This project was supported in part 
AFOSR MURI under award number FA9550-14-1-0351.
The authors would like to thank Dr Chung Lam, Dr Yu Zhu, Dr Simone Raoux, Dr Norma Sosa, Dr Matthew
BrightSky and Dr Adam Cywar for their contributions to device fabrication at IBM T.J. Watson Research Center.

==> Draft_eprint - Copy/sections/acknowledgment.tex <==
\section*{Acknowledgment}
%This project was supported in part by AFOSR MURI under award number FA9550-14-1-0351. 

The devices are fabricated at IBM T.J. Watson Research Center and characterized at UConn, supported by the U. S. National Science Foundation under awards number ECCS 0925973 and ECCS 1150960. The characterization and analysis efforts of R. S. Khan, N. Noor, J. Scoggin, H. Silva and A. Gokirmak and the problem statement and motivation of C. Jin, H. P. Nguyen and M. van Dijk are supported by AFOSR MURI under award number FA9550-14-1-0351. The authors would like to thank Dr. Chung Lam, Dr. Yu Zhu, Dr. Simone Raoux, Dr. Norma Sosa, Dr. Matthew BrightSky and Dr. Adam Cywar for their contributions to device fabrication at IBM T.J. Watson Research Center.

==> Draft_eprint - Copy/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%In this paper, we show that the variability of lithographic process can allow us to construct a reliable POK that is secure against physical attacks. In addition, we proposed a novel PCM-based POK which can achieve a reliable output based on the variability of granularity in PCM cells. Experimental results of lithography base POK and simulated results of PCM-based POKs are provided. 

We propose two new approaches for intrinsically reliable and lightweight POKs. One approach is based on utilizing the lithography limits to produce line cells that have random functionality. The second approach is a novel PCM-based POK which can achieve a reliable output based on the variability of granularity in PCM cells. Experimental results of lithography-based POK and simulated results of PCM-based POKs are provided.

==> Draft_eprint - Copy/sections/experiment.tex <==
\section{Experiment}
\label{sec:experiment}



==> Draft_eprint - Copy/sections/granularity.tex <==
\section{The Variability of Granularity of PCM}
\label{sec:granularity}



==> Draft_eprint - Copy/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

Since \textbf{Physical Unclonable Functions} (PUFs)~\cite{Pappu2001} were introduced in 2001, they have been considered as promising hardware security primitives for building secure systems such as IP protection, identification and authentication protocols, cryptographic primitives, etc.~\cite{Kumar2008,Armknecht2009,Maes2010,Yu2011,Brzuska2011}. 

PUFs exhibit a random challenge-response behavior, i.e., a random-looking response is generated by a PUF when queried with a specific challenge based on intrinsic manufacturing variations. All PUF behaviors are unique and \textit{physically unclonable}.

We partition PUF designs into two different categories: \textit{strong PUFs} and \textit{weak PUFs} (also called Physical Obfuscated Keys or POKs)~\cite{Gassend2003a}. The major difference between these two categories is that a strong PUF has a large number of challenge-response pairs (CRPs), while a weak PUF or POK has a limited number of CRPs. 

In this paper we focus on POKs, which due to its important security properties such as physical unclonability with tamper-resistance, uniqueness,  and unpredictability (or randomness) can be used for IP protection, authentication protocols~\cite{Suh2007}, tamper-resistant storage of random keys or building digital PUFs~\cite{Gassend2003a}.
% (see Figure~\ref{fig:DigitalPUF} and the detail of Figure~\ref{fig:DigitalPUF} is explained in Section~\ref{subsec:relibility_enhancement}). 
 For example, in the digital PUF concept a keyed Pseudo Random Function (PRF) is used as a PUF where challenges are inputs to the PRF and responses are the outputs of the PRF and where the key is a POK response of a fixed challenge to the POK.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/POK_DigitalPUF.pdf}
%\caption{Architecture of a physically obfuscated PUF in~\cite{Gassend2003a}}
%\label{fig:DigitalPUF}
%\end{figure}
%
%The first POK-based system was introduced as a \textit{digital PUF}~\cite{Gassend2003a} where the secret key of the system is the response to a fixed challenge.
%(see Figure~\ref{fig:DigitalPUF}). 
Since there is no secret key stored in non-volatile memory (NVM) in a POK-based system, the adversary cannot directly retrieve the secret key from the device. 

Typically, the POK circuit consists of two parts: a randomness source and a randomness extraction circuit. The randomness extraction circuit extracts and converts the analog signal from a randomness source into a response in the form of  \textbf{digital raw output} to be used in further digital computation. For example, in a Ring Oscillator (RO) based POK~\cite{Suh2007}, the randomness source is the delay randomness of circuit components  and the randomness extraction circuit consists of RO pairs with counters and comparators. For each RO pair its frequencies (measured by a counter) are compared (by a comparator)  to produce one bit raw output. The collection of the digital raw output bits from all RO pairs together forms the response of the POK. In this paper we consider POKs with just {\em one} challenge response pair, i.e., when powered-up a POK just (re)generates one fixed random looking response (after randomness extraction).

%Moreover, since POK's raw  outputs are tamper-resistant, the security of the system is enhanced in terms of tamper-resistance. In other words, 
One feature of a POK is that if an adversary physically opens the device for reverse engineering purpose, then the POK's randomness source and consequently raw output (i.e., response)  is changed. Therefore, if the POK's raw output is used as a secret key in a symmetric key system or as a key mask in public key systems, the adversary cannot physically open the device for retrieving such a secret key.  

%The following important properties of POK are studied for evaluating our proposed POK constructions:  
A POK design must offer POKs with the following properties:
\begin{itemize}
\item \textbf{Robustness/Reliability:}  The POK response is stable (i.e., the POK is able to regenerate the same response over and over).
\item  \textbf{Unpredictability:} The POK response is not predictable (without access to the POK), i.e., it should be randomly generated.
\item \textbf{Uniqueness:} A POK's response is different from device to device.
\end{itemize}
These properties are necessary in order for a POK response to be used as a key  in a secure system. In particular, a POK's response bits must be reliable and independent and identically distributed (i.i.d.) (i.e. not correlated). Both of these required properties may not immediately be satisfied for basic POK designs (such as the afore mentioned RO POK): To overcome the reliability and unpredictability problem, an Error Correcting Code (ECC)~\cite{Gassend2002a,Suh2007} with Privacy Amplification (PA) or Fuzzy Extractor (FE)~\cite{dodis2004fuzzy} is exploited to make a POK's (or more generally a PUF's) output robust and unpredictable. However, this approach leads to additional requirements in terms of \textbf{hardware overhead and efficiency}  as discussed in detail in Section~\ref{subsec:relibility_enhancement}. 

 



%\marten{for what?}
%\marten{what has PUF to do with the abstract? may be say ``since PUF and as a special class POKs were''}
%There are many proposed PUF designs, for example Arbiter PUFs (APUFs)~\cite{Lim2004}, Controlled PUFs~\cite{Gassend2002a}, Ring Oscillator PUFs (RO PUFs), XOR PUFs~\cite{Suh2007}, Lightweight Secure PUFs~\cite{Majzoobi2008a}, Composite PUFs~\cite{Sahoo2014} and LPN-based PUFs~\cite{HerderRenDijkEtAl2016}, Phase Change Memory based
%PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, etc. 
%\marten{above line can go to related work}
%Typically, PUFs exhibit a random challenge-response behavior, i.e., a random-looking response is generated by PUF when queried with a specific challenge based on intrinsic manufacturing variations. Since the PUFs is built based on the manufacturing process variation, all the PUFs are different and  \textit{physically unclonable}. 
%\marten{typically? I think always.  Do you mean different PUFs from the same PUF design are all different? We only assume that manufacturing variations cannot be physically cloned.}
%Due to the physically unclonable property, there is a large number of proposed applications which either complement or substitute traditional cryptographic algorithms~\cite{Kumar2008,Armknecht2009,Maes2010,Yu2011,Brzuska2011}.
%\marten{algorithms such as? -- may want to focus on what POKs are good for}
% In practice, we can partition all PUF designs into two different categories: \textit{strong PUF} and \textit{weak PUFs} (or Physically Obfuscated Keys - POKs)~\cite{Gassend2003a}. The major difference between those two categories is that the former has a large number of challenge-response pairs (CRPs), while the latter has a limited number of CRPs. In this paper, we focus on POKs.
% \marten{see above - why are these interesting?} For the POK, there are many properties \marten{what are the others? -- need to know this how else can we claim we design new POKs} and here three most important properties of POK are:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device. \marten{PUF to POK?}




  
  
% However, the presence of ECC can reduce the security of PUFs, i.e., the adversary can develop some attacks on PUFs~\cite{Delvaux2014,Nguyen2015} due to the presence of \textit{helper data} which is required for error correction process. \marten{Explain this reduction in security: You need to first explain that PA needs to be added because of the public helper data and that a hash of the corrected and amplified output should serve as a key (in PUF design for re-usability). You can give the example of a RO POK with 25\% noise under extreme temperature variations. One needs many POK output bits to get secure bits out. The question is also how does the helper data affect security? If one publishes many helper data for many responses, then in the PUF domain one can possibly break the PUF -- this is unknown. For POKs though we have just one helper data. And also we do not need the re-usability as for PUFs. So security is not reduced as for PUFs. Try to add this understanding by comparing the POK and PUF.} Moreover, using ECC has to pay a high cost in terms of hardware overhead, implementation efficiency as pointed in~\cite{BhargavaMai2013}. As an important note, the ECC-based approach only works if certain conditions are satisfied (see Fuzzy Extractor~\cite{dodis2004fuzzy}). \marten{It is better to indicate that the ECC approach with PA combined us what is now called FE. Best is to mention this earlier upfront. } \marten{If this is an important note, then you should explain these certain conditions -- and why this is important ! It now reads like an empty statement.}

We notice an alternative approach for a POK/PUF design based on bi-stable memories (for example SRAM memory) for which  the reliability of the POK/PUF output can be significantly improved by output reinforcement processes as discussed in~\cite{BhargavaCakirMai2012,BhargavaMai2013}, for example, by the Hot Carrier Injection technique. Typically, this process changes the POK/PUF's circuit characteristics permanently and thus the POK/PUF's output can be highly reliable. To achieve this goal, however, a suitable setup is required.
%(\textcolor{red}{Ha: Chenglu and Nafisa can you verify this claim?}) and it is not always available to the PUF designer. It is %evident that reinforcement processes increase the manpower and technology efforts for PUF design. 
%Compared to the ECC-based approach,  response reinforcement is not general and only applies to bi-stable memories. 

% as shown in~\cite{BhargavaCakirMai2012,BhargavaMai2013}. \marten{You should write ``For PUF design based on bi-stable memeories the reliability of the PUF output can be significantly ...'' at the start of the paragraph and delete this sentence.}
%
%For the ECC-based approach, to solve the i.i.d. problem, \marten{What is the iid problem? It was not explained earlier? Is it a problem? It becomes a problem if one feels that for correlated noise one implicitly needs to assume a computational hardness assumption which states that the FE approach also is secure with respect to such noise in that the correlations can not be computationally exploited. A sentence like this can be part of an earlier paragraph were you explain realiability, FE, helper data etc.} the raw output of POK after the error correction process must go through a \textit{privacy amplification process} which requires \textbf{a true random bit string} (see Fuzzy Extractors~\cite{dodis2004fuzzy}). \marten{input string? As you can see a bunch of my comments and text spread out in these paragraphs can be re-organized in a better logical order.} Actually, we have the following major challenges for using FEs for de-correlating POK's outputs: \marten{Actually? You like to now enumerate the challenges because you have explained the whole reliability problem in sufficient detail.}
%\begin{enumerate}
%\item \textbf{Security.} Since it is required to quantify the min-entropy of the raw POK's output for computing the final output of FEs and this is a \textit{impossible} mission in practice due to the large number of POK's output bits and its correlation, we cannot exactly address the security of POK-based system in the presence of FEs. \marten{Suggestion: Use separate paragraph headings such as ``security'' so that the above comments/text clearly explain what is happening.}
%\item \textbf{Hardware overhead.} The hardware footprint is significantly increased due to the presence of true random bit string.
%\marten{This is out of the blue. You need to explain FE using a picture and give enough details to explain where the TRNG comes in and why.}
%\item \textbf{Efficiency.} The efficiency of the POK-based systems is significantly reduced due to the use of hash function in FEs.   \marten{Again what is going on? You mean the PA implemented by the hash function reduces the rate of amount of secret output bit per POK bit.}
%\end{enumerate}
%\marten{I think we need a separate (sub?)section on reliability with a bunch of the above clearly cristalized in that section. The intro just gives a brief heads up with the main conclusion of that section.}

In this paper we search for other alternative and practical POK designs that allow a (basic) randomness extraction circuit which does not need any ECC circuitry because the randomness source of the POK itself is intrinsically reliable such that a simple comparator based solution produces bits that are both reliable and as a collective have high min-entropy. Due to having a high min-entropy, the de-correlation problem (making the final response i.i.d.)  can be solved in a simple way by using the de-correlation technique from True Random Number Generator (TRNG) constructions, where typically several bits are XORed together resulting in i.i.d. response bits. This leads to lightweight POK designs without expensive ECC and PA circuitry. 

%  the constructed bit is not biased and the independence and identically distribution property between the constructed bits are enhanced. Hence, we can solve the long term open and fundamental problem in PUF's research topic with a lightweight XOR-based network. 
  
If it is possible to design \textit{intrinsically} reliable POKs based on common technology  without needing a specialized set-up per fabricated POK, then no reliability enhancement techniques are needed and resulting in lightweight POK designs as explained above. We propose two new intrinsically reliable POK designs:
%In other words, our POK design includes a raw reliable POK output and XOR-based network. Since, the POK's outputs are i.i.d, then all systems which are based on this POK can be \textbf{provably secure}. Note that, \textit{provable security} is also long-term fundamental problem in hardware security (see Section~\ref{subsec:relibility_enhancement}).

%\marten{This paragraph is the core motivation and should be stressed as such -- let's push the whole reliability discussion out to a next section ``Reliability Enhancement and Related Work''}

%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/UNOPOK.pdf}
%\caption{Difference between UNO and POK/PUF}
%\label{fig:unopok}
%\end{figure}

\vspace{3mm}

\noindent
\textbf{POK based on the Variability of Lithographic Process:}
%In this paper, our main contributions are as follows. 
First, we observe that a lithographic process can provide a good random source if applied below the particular process limit. Typically, the lithographic process can be used to create a \textbf{Unique Object (UNO)}~\cite{Ruhrmair2011}. In~\cite{Ruhrmair2011}, a UNO is described as  ``A physical system that, upon measurement by an external apparatus, exhibits a small, fixed set of inimitable analog properties that are not similar to any other objects.'' A UNO is different from a POK in the way we measure the objects. For a POK, we have to use an internal apparatus so as to not expose the output while UNO's output is measured by an external aparatus and is not kept as a secret. As an important property, the output of a UNO is intrinsically reliable.
% Figure~\ref{fig:unopok} shows the difference between the notions UNO and POK/PUF.

%\marten{Let's explain this in a picture and put this definition upfront where POK/PUF is explained. Here we can refer to the picture again and explain where the two solutions fall. The picture also indicates the noise problem, i.e. UNO is generally perfectly reliable and POK/PUF not and we push this boundary.}



%Typically, the wires (connections) in a chip can be randomly connected or disconnected if we force the lithographic process to work with very small scales. This property is called \textbf{variability of lithographic process}. 
Typically, the smallest features on a chip are safely above the lithographic process limit to ensure a high yield. But features at this limit can be exploited to obtain a random array of functional/broken devices. Hence, the connectivity of each such line cell can be converted to a random bit. This means  a secret key or a key mask based on the connectivity of cells can be constructed in a robust way. 
%Moreover, this secret key / key mask can be generated in reliable way. 
%
%\marten{You mean random secret key -- may be we should use ``random mask'' which is used to XOR the actual secret key with, there sult stored in non-volatile memory -- see the digital PUF picture. By the way a digital PUF hardcodes a key as POK from which a PUF is derived. } 

Notice that a set of line cells constructed by a lithographic process is a UNO, however, if this set is hidden, then we obtain a POK instead of a UNO. 
%We will show that, if the adversary physically accesses the set of wires in the chip, then the connectivity of wires is not clearly visible. 
Since the width of cells is very small, we can have many random bits giving a high density key. 

%\marten{Confusing. I thought it is about the external measurement apparatus. We can say that our solution is like a UNO in that it is noise-free.} 

In PUF literature, the lithographic process has been introduced to construct PUF designs as shown in~\cite{SreedharKundu2011,KumarBurleson2013,KumarDhanuskodiKundu2014}, see Section \ref{subsec:lithoPUF}. However, our proposed design based on connectivity is very reliable and requires minimal randomness extraction circuitry.
%\marten{Either to related work, or consistently add such a paragraph for our second PCM solution.}

%However, if the adversary can physically access the device to observe the connectivity of wires, then the security of this random string is not guaranteed anymore. 

\vspace{3mm}

\noindent
\textbf{POK based on the Variability of Granularity in Phase Change Memory:}
As a second contribution, we propose a novel Phase Change Memory (PCM) based POK. Existing PCM-based PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} compare resistances of two PCM cells which differ due to process variation in order  to produce one output bit. The resistances are not reliable due to resistance fluctuations over time. Our proposed PCM-based POK differs from those in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} in terms of design concept. We use a single PCM device with three contacts to produce one bit based on \textbf{grain map variability in the PCM device}. Our proposed PCM cell randomly programs one of two contacts, thus a 0 or 1 is encoded. We can achieve a reliable PCM-based POK without using any reliability-enhancement techniques as mentioned above.  
 
% Compared to the method based on lithographic process, since no-one can physically observe the granularity inside the PCM cell, the proposed PCM-based POK is secure against physical attacks. 

\vspace{3mm}

\noindent
\textbf{Organization:}
%The rest of paper is organized as follows. 
We discuss related works in Section~\ref{sec:notation_background}. Section~\ref{sec:lithography} presents the lithography-based POK. The PCM-based POK is described in Section~\ref{sec:pcm}. Section~\ref{sec:conclusion} concludes this paper. 
 



%In addition, the helper data is required and it is stored off-chip in non-volatile memories which is later used for correcting the errors in PUF's raw outputs.


 

%UNO~\cite{Ruhrmair2011}
%
%Digital PUF was first introduced in~\cite{Gassend2003a}
%
%In~\cite{Tuyls2006}, Tuyls et al. proposed a PUF design which has a single pair of challenge-response. 
%Actually, the response is used as cryptographic key and any attempts to breach the device will destroy the key. 
%This kind of system provides read-proof key storage, and is called as a weak PUF~\cite{Guajardo2007,Ruhrmair2009a} or 
%physically obfuscated key (POK)~\cite{Gassend2003}. A strong PUF has many CRPs and the adversary may access a set of CRPs but cannot sample exhaustively. However, POK has few CRPs and thus, as the security requirement, the CRPs must remain secret from the adversary. 
%
%For the POK, there are many properties and here three most important properties of POK are:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device
%
%% \textcolor{red}{Ha: how we can measure the uniqueness of proposed PCM-based POK?}.  
%
%One of the major research topics in PUFs is achieving a highly reliable PUF's responses or outputs. Since PUFs implementation is based on intrinsic manufacturing variations, the PUF behavior may be slightly different each time when the environmental conditions (e.g, temperature, supplying voltage) change~\cite{Lim2004}. To cope this problem, Error Correction Code (ECC)~\cite{Gassend2002a,Suh2007} or Fuzzy Extractor~\cite{dodis2004fuzzy} is exploited to make PUF's output stable. However, the presence of ECC can reduce the security of PUFs, i.e., the adversary can develop some attacks on PUFs~\cite{Delvaux2014,Nguyen2015}. Moreover, using ECC has to pay a high cost in terms of hardware overhead, implementation efficiency as pointed in~\cite{BhargavaMai2013}. In addition, the helper data is required and it is stored off-chip in non-volatile memories which is later used for correcting the errors in PUF's raw outputs. 
%
%As an alternative approach, the reliability of PUF's output can be significantly improved by reinforcement process as discussed in~\cite{BhargavaCakirMai2012,BhargavaMai2013}. Typically, this process will permanently change the PUF's circuit characteristic and thus, the PUF's output can be highly reliable. To achieve this goal, the special instrument is required (Chenglu can you verify this claim?) and it is not always available for the PUF designer.
%
%In recent years, it is shown that Phase Change Memories (PCMs) can be used to construct PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}. PCM is a nanoscale non-volatile memory and it has a good aging-resistance property. However, the output of PCM-based PUFs is not reliable as shown in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}. 
%Thus, if PCM is used to construct POK, then ECC or reinforcement process are in need. 
%
%In this paper, our main constructions are as follows. First, we observe that the lithographic process can provide a good random source in case of nano-scale technology. Typically, the wires (connections) in the devices can be randomly connected or disconnected if we force the lithographic process work with very small scales. This property is called as \textit{variability of lithographic process}. Hence, the connectivity of wires in devices can be converted as a random bit string which can be used as secret key (POK) in secure protocols. Moreover, this random string can be generated in reliable way. However, if the adversary can physically access the device to observe the connectivity of wires, then the security of this random string is not guaranteed anymore. As a second contribution, we propose a novel PCM-based POK. In the existing PCM-based PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, the resistances of two PCM cells, which are randomly defined by the process variation, are compared to produce a output bit. Due to the fluctuation in the current, the resistances can be changed and thus, the output is not reliable. Our proposed PCM-based POK is different from that in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} in terms of architecture, i.e., we use only one PCM cell to produce one bit output based on \textbf{the variability of granularity of PCM cells}. Thus, we can achieve a reliable PCM-based POK without using any reliability-enhancement techniques as mentioned above. Compared to the method based on lithographic process, since no-one can physically observe the granularity inside the PCM cell, the proposed PCM-based POK is secure against physical attacks. 
%
%The rest of the paper is organized as follows. We discuss related work in Section~\ref{sec:notation_background}. Section~\ref{sec:conclusion} concludes this paper. 

==> Draft_eprint - Copy/sections/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Since \textbf{Physical Unclonable Functions} (PUFs)~\cite{Pappu2001} were introduced in 2001, they have been considered as promising hardware security primitives for building secure systems such as IP protection, authentication protocol, cryptographic primitives, etc~\cite{Kumar2008,Armknecht2009,Maes2010,Yu2011,Brzuska2011}. 

PUFs exhibit a random challenge-response behavior, i.e., a random-looking response is generated by PUF when queried with a specific challenge based on intrinsic manufacturing variations. Since the PUFs is built based on the manufacturing process variation, all the PUF's behavior is unique and \textit{physically unclonable}.

In practice, we can partition all PUF designs into two different categories: \textit{strong PUF} and \textit{weak PUFs} (or Physically Obfuscated Keys - POKs)~\cite{Gassend2003a}. The major difference between those two categories is that the former has a large number of challenge-response pairs (CRPs), while the latter has a limited number of CRPs. In this paper, we focus on POKs. POKs can be used for IP protection, authentication protocol~\cite{Suh2007}, tamper-resistant storage of random keys or building digital PUFs~\cite{Gassend2003a} due to its important security properties such as physical unclonability, uniqueness, tamper-resistance, unpredictability (or randomness), etc. In this paper, we focus on the following important properties of POK for evaluating our proposed POK constructions:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device.

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/POK_DigitalPUF.pdf}
\caption{Architecture of a physically obfuscated PUF in~\cite{Gassend2003a}}
\label{fig:DigitalPUF}
\end{figure}

The first POK-based system was introduced as a \textit{digital PUFs}~\cite{Gassend2003a} where the secret key of the secure systems is the response of a fixed challenge (see Figure~\ref{fig:DigitalPUF}). Since there is no secret key stored in a non-volatile memory (NVM) in POK-based system, the adversary cannot directly retrieve the secret key from the device. 

Typically, the POK circuit consists of two parts: randomness source and randomness extraction circuit. The randomness extraction circuit extracts and converts the analog signal from randomness source into \textbf{the raw output (digital signal)} which can be used in digital systems. For example, in RO-based POK~\cite{Suh2007}, the randomness source is the delay randomness in each circuit component,  and randomness extraction circuit are Ring Oscillators (ROs), counter and comparator. A pair of ROs is chosen and their frequencies (measured by counter) are compared to each other to procedure one bit output. 

Moreover, since the raw POK's outputs are tamper-resistant, the security of system is enhanced in term of tamper-resistance. In other words, if the adversary physically opens the device for reverse engineering purpose, then the raw POK's outputs are changed. Hence, if the raw POK's outputs are used as a secret key in symmetric key system or as a key mask in public key systems, the adversary cannot physically open the device for retrieving the secrets.  

However, to be used in secure systems, the raw POK outputs and \textit{independent and identically distributed-i.i.d.} (i.e. not correlated). Both of those required properties are not satisfied for raw POK outputs. To over come the reliability problem, Error Correction Code (ECCs)~\cite{Gassend2002a,Suh2007} or Fuzzy Extractor~\cite{dodis2004fuzzy} is exploited to make PUF's output stable. However, we have to face with many challenges in terms of \textbf{security, hardware overhead and efficiency} when the ECC is applied to enhance the reliability of POK as discussed in detail in Section~\ref{subsec:relibility_enhancement}. 

 



%\marten{for what?}
%\marten{what has PUF to do with the abstract? may be say ``since PUF and as a special class POKs were''}
%There are many proposed PUF designs, for example Arbiter PUFs (APUFs)~\cite{Lim2004}, Controlled PUFs~\cite{Gassend2002a}, Ring Oscillator PUFs (RO PUFs), XOR PUFs~\cite{Suh2007}, Lightweight Secure PUFs~\cite{Majzoobi2008a}, Composite PUFs~\cite{Sahoo2014} and LPN-based PUFs~\cite{HerderRenDijkEtAl2016}, Phase Change Memory based
%PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, etc. 
%\marten{above line can go to related work}
%Typically, PUFs exhibit a random challenge-response behavior, i.e., a random-looking response is generated by PUF when queried with a specific challenge based on intrinsic manufacturing variations. Since the PUFs is built based on the manufacturing process variation, all the PUFs are different and  \textit{physically unclonable}. 
%\marten{typically? I think always.  Do you mean different PUFs from the same PUF design are all different? We only assume that manufacturing variations cannot be physically cloned.}
%Due to the physically unclonable property, there is a large number of proposed applications which either complement or substitute traditional cryptographic algorithms~\cite{Kumar2008,Armknecht2009,Maes2010,Yu2011,Brzuska2011}.
%\marten{algorithms such as? -- may want to focus on what POKs are good for}
% In practice, we can partition all PUF designs into two different categories: \textit{strong PUF} and \textit{weak PUFs} (or Physically Obfuscated Keys - POKs)~\cite{Gassend2003a}. The major difference between those two categories is that the former has a large number of challenge-response pairs (CRPs), while the latter has a limited number of CRPs. In this paper, we focus on POKs.
% \marten{see above - why are these interesting?} For the POK, there are many properties \marten{what are the others? -- need to know this how else can we claim we design new POKs} and here three most important properties of POK are:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device. \marten{PUF to POK?}




  
  
% However, the presence of ECC can reduce the security of PUFs, i.e., the adversary can develop some attacks on PUFs~\cite{Delvaux2014,Nguyen2015} due to the presence of \textit{helper data} which is required for error correction process. \marten{Explain this reduction in security: You need to first explain that PA needs to be added because of the public helper data and that a hash of the corrected and amplified output should serve as a key (in PUF design for re-usability). You can give the example of a RO POK with 25\% noise under extreme temperature variations. One needs many POK output bits to get secure bits out. The question is also how does the helper data affect security? If one publishes many helper data for many responses, then in the PUF domain one can possibly break the PUF -- this is unknown. For POKs though we have just one helper data. And also we do not need the re-usability as for PUFs. So security is not reduced as for PUFs. Try to add this understanding by comparing the POK and PUF.} Moreover, using ECC has to pay a high cost in terms of hardware overhead, implementation efficiency as pointed in~\cite{BhargavaMai2013}. As an important note, the ECC-based approach only works if certain conditions are satisfied (see Fuzzy Extractor~\cite{dodis2004fuzzy}). \marten{It is better to indicate that the ECC approach with PA combined us what is now called FE. Best is to mention this earlier upfront. } \marten{If this is an important note, then you should explain these certain conditions -- and why this is important ! It now reads like an empty statement.}

For PUF design based on bi-stable memories the reliability of the PUF output can be significantly improved by output reinforcement process as discussed in~\cite{BhargavaCakirMai2012,BhargavaMai2013}, for example Hot Carrier Injection technique. Typically, this process changes the PUF's circuit characteristic permanently and thus, the PUF's output can be highly reliable. To achieve this goal, a suitable setup is required (\textcolor{red}{Ha: Chenglu and Nafisa can you verify this claim?}) and it is not always available to the PUF designer. It is evident that reinforcement process increases the manpower and technology efforts for PUF design. In additional, compared to the ECC-based approach, the response reinforcement is not general, i.e., it is only available to bi-stable memories. 

% as shown in~\cite{BhargavaCakirMai2012,BhargavaMai2013}. \marten{You should write ``For PUF design based on bi-stable memeories the reliability of the PUF output can be significantly ...'' at the start of the paragraph and delete this sentence.}
%
%For the ECC-based approach, to solve the i.i.d. problem, \marten{What is the iid problem? It was not explained earlier? Is it a problem? It becomes a problem if one feels that for correlated noise one implicitly needs to assume a computational hardness assumption which states that the FE approach also is secure with respect to such noise in that the correlations can not be computationally exploited. A sentence like this can be part of an earlier paragraph were you explain realiability, FE, helper data etc.} the raw output of POK after the error correction process must go through a \textit{privacy amplification process} which requires \textbf{a true random bit string} (see Fuzzy Extractors~\cite{dodis2004fuzzy}). \marten{input string? As you can see a bunch of my comments and text spread out in these paragraphs can be re-organized in a better logical order.} Actually, we have the following major challenges for using FEs for de-correlating POK's outputs: \marten{Actually? You like to now enumerate the challenges because you have explained the whole reliability problem in sufficient detail.}
%\begin{enumerate}
%\item \textbf{Security.} Since it is required to quantify the min-entropy of the raw POK's output for computing the final output of FEs and this is a \textit{impossible} mission in practice due to the large number of POK's output bits and its correlation, we cannot exactly address the security of POK-based system in the presence of FEs. \marten{Suggestion: Use separate paragraph headings such as ``security'' so that the above comments/text clearly explain what is happening.}
%\item \textbf{Hardware overhead.} The hardware footprint is significantly increased due to the presence of true random bit string.
%\marten{This is out of the blue. You need to explain FE using a picture and give enough details to explain where the TRNG comes in and why.}
%\item \textbf{Efficiency.} The efficiency of the POK-based systems is significantly reduced due to the use of hash function in FEs.   \marten{Again what is going on? You mean the PA implemented by the hash function reduces the rate of amount of secret output bit per POK bit.}
%\end{enumerate}
%\marten{I think we need a separate (sub?)section on reliability with a bunch of the above clearly cristalized in that section. The intro just gives a brief heads up with the main conclusion of that section.}

We \textbf{observe} that if the raw POK's output is reliable, then the de-correlation problem  can be solved in the simple way by using the de-correlation technique from the construction of True Random Number Generation. Typically, if we XOR many correlated bits together, the constructed bit is not biased and the independence and identically distribution property between the constructed bits are enhanced. Hence, we can solve the long term open and fundamental problem in PUF's research topic with a lightweight XOR-based network. Thus, the main question is that \textit{can we have intrinsically reliable POK design?}. If possible, then all the problems related to the reliability enhancement technique will be dropped. In other words, our POK design includes a raw reliable POK output and XOR-based network. Since, the POK's outputs are i.i.d, then all systems which are based on this POK can be \textbf{provably secure}. Note that, \textit{provable security} is also an long-term fundamental problem in hardware security research topic (see Section~\ref{subsec:relibility_enhancement}).

\marten{This paragraph is the core motivation and should be stressed as such -- let's push the whole reliability discussion out to a next section ``Reliability Enhancement and Related Work''}

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/UNOPOK.pdf}
\caption{Difference between UNO and POK/PUF}
\label{fig:unopok}
\end{figure}

\textbf{Contributions.}
In this paper, our main contributions are as follows. First, we observe that the lithographic process can provide a good random source in case of nano-scale technology. Typically, the lithographic process can be used to create \textbf{Unique Object - UNO}~\cite{Ruhrmair2011}. In~\cite{Ruhrmair2011}, the UNO is described as  ``A Unique Object is a physical system that, upon measurement by an external apparatus, exhibits a small, fixed set of inimitable analog properties that are not similar to any other objects''. In rough words, UNO is different from POK in the way we measure the objects. For POK, we have to use the internal apparatus to not expose the output of POK and UNO's output is not kept as secret. As an important property, the output of UNO is reliable. Figure~\ref{fig:unopok} shows the difference between the notions UNO and POK/PUF.

%\marten{Let's explain this in a picture and put this definition upfront where POK/PUF is explained. Here we can refer to the picture again and explain where the two solutions fall. The picture also indicates the noise problem, i.e. UNO is generally perfectly reliable and POK/PUF not and we push this boundary.}

Typically, the wires (connections) in a chip can be randomly connected or disconnected if we force the lithographic process to work with very small scales. This property is called as \textbf{variability of lithographic process}. Hence, the connectivity of each such wire can be converted to a random bit. Hence, a secret key/ a key mask based on the connectivity of wires can be constructed in secure protocols. Moreover, this secret key / key mask can be generated in reliable way. 

%\marten{You mean random secret key -- may be we should use ``random mask'' which is used to XOR the actual secret key with, there sult stored in non-volatile memory -- see the digital PUF picture. By the way a digital PUF hardcodes a key as POK from which a PUF is derived. } 

Specifically, a set of wires constructed by lithographic process is UNO but if this set is hidden, then we have POK instead of UNO. We will show that, if the adversary physically access the set of wires in the chip, then the connectivity of wires is changed, i.e., we have a tamper-resistant and reliable POK design. Since the width of wires is pretty small, we can have many random bits in a significantly small hardware footprint. \footnote{Needs to be checked by Ali/Helena etc.}

%\marten{Confusing. I thought it is about the external measurement apparatus. We can say that our solution is like a UNO in that it is noise-free.} 

In the PUF's literature, the lithographic process has been introduced to construct PUF designs as shown in~\cite{SreedharKundu2011,KumarBurleson2013,KumarDhanuskodiKundu2014}. However, the design philosophy of PUF designs in those papers is different (i.e., not use the connectivity of the wires) and the PUF's outputs are not reliable.  
%\marten{Either to related work, or consistently add such a paragraph for our second PCM solution.}

%However, if the adversary can physically access the device to observe the connectivity of wires, then the security of this random string is not guaranteed anymore. 

As a second contribution, we propose a novel Phase Change Memory (PCM) based POK. In the existing PCM-based PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, the resistances of two PCM cells, which are randomly defined by the process variation, are compared to produce a output bit. Due to the fluctuation in the current, the resistances can be changed and thus, the output is not reliable. Our proposed PCM-based POK is different from that in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} in terms of design philosophy, i.e., we use only one PCM cell to produce one bit output based on \textbf{the variability of granularity of PCM cells}. Our proposed PCM cell is randomly programmed as a ``left'' or ``right'' gate through which reliably a 0 or 1 is encoded. Thus, we can achieve a reliable PCM-based POK without using any reliability-enhancement techniques as mentioned above.  

To support all proposed theoretical results, we demonstrate the simulations and experiments in detail. 

% Compared to the method based on lithographic process, since no-one can physically observe the granularity inside the PCM cell, the proposed PCM-based POK is secure against physical attacks. 

The rest of paper is organized as follows. We discuss related work in Section~\ref{sec:notation_background}. Section~\ref{sec:lithography} presents the lithography based POK. The PCM-based POK is described in Section~\ref{sec:granularity}. Section~\ref{sec:experiment} demonstrates the simulated results on lithography and PCM based POKs. Section~\ref{sec:conclusion} concludes this paper. 
 



%In addition, the helper data is required and it is stored off-chip in non-volatile memories which is later used for correcting the errors in PUF's raw outputs.


 

%UNO~\cite{Ruhrmair2011}
%
%Digital PUF was first introduced in~\cite{Gassend2003a}
%
%In~\cite{Tuyls2006}, Tuyls et al. proposed a PUF design which has a single pair of challenge-response. 
%Actually, the response is used as cryptographic key and any attempts to breach the device will destroy the key. 
%This kind of system provides read-proof key storage, and is called as a weak PUF~\cite{Guajardo2007,Ruhrmair2009a} or 
%physically obfuscated key (POK)~\cite{Gassend2003}. A strong PUF has many CRPs and the adversary may access a set of CRPs but cannot sample exhaustively. However, POK has few CRPs and thus, as the security requirement, the CRPs must remain secret from the adversary. 
%
%For the POK, there are many properties and here three most important properties of POK are:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device
%
%% \textcolor{red}{Ha: how we can measure the uniqueness of proposed PCM-based POK?}.  
%
%One of the major research topics in PUFs is achieving a highly reliable PUF's responses or outputs. Since PUFs implementation is based on intrinsic manufacturing variations, the PUF behavior may be slightly different each time when the environmental conditions (e.g, temperature, supplying voltage) change~\cite{Lim2004}. To cope this problem, Error Correction Code (ECC)~\cite{Gassend2002a,Suh2007} or Fuzzy Extractor~\cite{dodis2004fuzzy} is exploited to make PUF's output stable. However, the presence of ECC can reduce the security of PUFs, i.e., the adversary can develop some attacks on PUFs~\cite{Delvaux2014,Nguyen2015}. Moreover, using ECC has to pay a high cost in terms of hardware overhead, implementation efficiency as pointed in~\cite{BhargavaMai2013}. In addition, the helper data is required and it is stored off-chip in non-volatile memories which is later used for correcting the errors in PUF's raw outputs. 
%
%As an alternative approach, the reliability of PUF's output can be significantly improved by reinforcement process as discussed in~\cite{BhargavaCakirMai2012,BhargavaMai2013}. Typically, this process will permanently change the PUF's circuit characteristic and thus, the PUF's output can be highly reliable. To achieve this goal, the special instrument is required (Chenglu can you verify this claim?) and it is not always available for the PUF designer.
%
%In recent years, it is shown that Phase Change Memories (PCMs) can be used to construct PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}. PCM is a nanoscale non-volatile memory and it has a good aging-resistance property. However, the output of PCM-based PUFs is not reliable as shown in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}. 
%Thus, if PCM is used to construct POK, then ECC or reinforcement process are in need. 
%
%In this paper, our main constructions are as follows. First, we observe that the lithographic process can provide a good random source in case of nano-scale technology. Typically, the wires (connections) in the devices can be randomly connected or disconnected if we force the lithographic process work with very small scales. This property is called as \textit{variability of lithographic process}. Hence, the connectivity of wires in devices can be converted as a random bit string which can be used as secret key (POK) in secure protocols. Moreover, this random string can be generated in reliable way. However, if the adversary can physically access the device to observe the connectivity of wires, then the security of this random string is not guaranteed anymore. As a second contribution, we propose a novel PCM-based POK. In the existing PCM-based PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, the resistances of two PCM cells, which are randomly defined by the process variation, are compared to produce a output bit. Due to the fluctuation in the current, the resistances can be changed and thus, the output is not reliable. Our proposed PCM-based POK is different from that in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} in terms of architecture, i.e., we use only one PCM cell to produce one bit output based on \textbf{the variability of granularity of PCM cells}. Thus, we can achieve a reliable PCM-based POK without using any reliability-enhancement techniques as mentioned above. Compared to the method based on lithographic process, since no-one can physically observe the granularity inside the PCM cell, the proposed PCM-based POK is secure against physical attacks. 
%
%The rest of the paper is organized as follows. We discuss related work in Section~\ref{sec:notation_background}. Section~\ref{sec:conclusion} concludes this paper. 

==> Draft_eprint - Copy/sections/lithography.tex <==
\section{Physical Obfuscated Key Based on Lithography Limit}
\label{sec:lithography} 



\begin{figure}[!t]
\centering
%\includegraphics[width = 0.6\columnwidth , height= 0.33\columnwidth]{./figs/sem_cell_trial}
\includegraphics[width = 0.4\columnwidth ]{./figs/sem_cell_}

\caption{SEM image of (a) connected cell, (b) broken cell, (c) cell with a void formed at the center.}
\vspace{-1 em}
\label{fig:sem_cell}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width = 0.8\columnwidth]{./figs/GST.png}
\caption{Illustration of GST line cell fabrication steps (a) 700 nm $SiO_2$ growth, (b) 250 nm deep trench formation, (c) 300 nm TiN fill, (d) chemical mechanical planarization (CMP), (e) GST film deposition (50 nm), (f) patterning of GST film, (g) $Si_3N_4$ cap layer deposition, (h) SEM image of a fabricated line cell~\cite{DirisaglikBakanJuradoEtAl2015}. }
\vspace{-1 em}
\label{fig:fab_cell}
\end{figure}\


%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/total_new}
%\caption{Connectivity yield color map for two-contact cells  with widths below the lithography limit (90 nm technology).Each block represents a group of line cells with similar design length and width. The width of the cells varies from group to group by 2nm (y axis) and length varies by 10 nm (x axis). The colors represent percentage of line cells that are functional in a group consisting of 10 cells of same design dimensions (e.g. yellow corresponds to size blocks where 5 out of the 10 cells are working/connected). The 40-60\% region of cell dimensions can be used to generate random, unique security keys. A yield map needs to be obtained for a given fabrication technology process.}
%\label{fig:litho_width}
%\end{figure}

%\subsection{Device Fabrication}
%The GST line cells used in the experiment were fabricated using the following procedure: 700 nm  Silicon Dioxide ($SiO_2$) was thermally grown on Silicon wafers. TiN contacts were made by making deep trenches (250 nm) in $SiO_2$ using optical lithography and reactive ion etching (RIE). The trenches were filled with TiN using chemical vapor deposition (CVD) and then polished to ensure uniform surface. 50 nm undoped GST was sputtered followed by a 10 nm $SiO_2$ cap deposition. The GST line cells were then patterned using optical lithography and RIE. Finally a 15 nm silicon nitride ($Si_3N_4$) blanket layer is deposited to encapsulate the structures~\cite{DirisaglikBakanJuradoEtAl2015}. The cells were annealed to 675K to ensure that they were in HCP state with minimum voids~\cite{BoZhi-TangSong-LinEtAl2004}. Illustration of GST line cells fabrication steps is presented in Figure~\ref{fig:GST}. 
%
%\subsection{Experimental Procedure} 
%The electrical measurements were performed at room temperature using Agilent 4156C Precision Semiconductor Parameter Analyzer. Small voltage (0.1V DC sweep) was used to perform the read operation in order to preserve the integrity of the cells.
%
%\subsection{Results}
%Measurements were made on GST line cells with design width varying from 40 nm to 60 nm and length varying from 340 nm to 500 nm. It was found out that for some dimensions, the cells were always functional and for some dimensions cells were always broken (see Figure~\ref{fig:litho_width}). It was found out that for some dimensions, the cells were always functional and for some dimensions cells were always broken. When the length of the line cells is short (i.e. 340 nm), the contacts of the line cells influence the width of the actual line cell . This causes the width of the line cell to be greater than its design width. So, these devices are always functional. But as the length increases, the effects of the contacts become less dominant. On the other hand, when the cell is long (i.e. 500 nm), the high exposure of light causes a break in the cell.   But in between these two extremes, there is a range where the possibility of having a functional cell is random. For examples, in line cells with design width and length of 50 nm and 420 nm respectively, 50 percent of the cells were functional while 50 percent were broken. Cells within this range can be used as bits in a string to authenticate a device, with a functional and broken wire representing 1 and 0 respectively. That way each device will have a secret key of its own, thereby forming a physically obfuscated key (POK). 
%
%By increasing the number of line cells to authenticate a device, brute force attacks will become difficult for the attacker. Also, the line cells used in the experiment have bottom contacts. So, the probability of an invasive attacker destroying GST is high. 
%
%Since process variations are process and machinery dependant, it would not be possible to reproduce the same bit strings in a different setup. This makes the device immune from cloning.
%
%A major drawback of this type of POK is that if the attacker manages to image the device using SEM without breaking the GST, the key will be revealed. So, additional circuitry is needed for improved security.
%
%Since the hexagonal phase is stable and the resistances of GST line cells are stochastic in nature due to process variation, another approach can be to use the resistance of the line cells to authenticate a device. Figure ? shows the resistances of GST line cells in a die varying from A to B. The whole range can be quantized into smaller ranges and each range can be assigned certain bits.
%
%
%\textcolor{red}{Ha: We need argument from Prof. Ali why it is tamper-resistant}

%\marten{Needs some intro: The section starts quite abruptly about ``the'' experiment.}

As shown in~\cite{BhargavaMai2013}, a reliable SRAM POK can be made by applying a response reinforcement technique. However, to produce one raw bit secret,  6 transistors are needed, i.e., one SRAM cell. Moreover, SRAM POK is feasible only when the device has SRAM as memory. Our approach can produce one raw bit secret at the cost of 1 transistor and one line cell (very small compared to the transistor), and our POK can be implemented in \textbf{any} device. 


For high-yield, reliable applications the smallest dimensions should be safely above the lithographic resolution limit at which some devices are successfully printed and others are not (Figure~\ref{fig:sem_cell}). For a given lithography process, the yield can be varied between 0\% and 100\% for devices with sizes well below the resolution limit and 100\% for devices with sizes well above the resolution limit. In this work we propose to use `lithography-limit' devices to implement true, physical randomness as connected or disconnected lines in a dense array of two contact devices. In this work, GST line cells are used to demonstrate the proof of concept, but the same idea can be applied to other materials (e.g. silicon, metal) to produce  a reliable POK.

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/total_new_}
\caption{{Connectivity yield color map for two-contact line cells  with widths below the lithography limit (90 nm technology) for 10 dies ($\thicksim$1870 devices). Each block represents a group of line cells with similar design length and width. The width of the cells varies from group to group by 2nm (y axis) and length varies by 10 nm (x axis). The colors represent percentage of line cells that are functional in a group consisting of 10 cells of same design dimensions (e.g. yellow corresponds to size blocks where 4 to 6 out of the 10 cells are working/connected). The 40-60\% region of cell dimensions can be used to generate random, unique security keys. A yield map needs to be obtained for a given fabrication technology process which will vary depending on fabrication parameters.}}
\vspace{-1 em}
\label{fig:litho_width}
\end{figure}

The bottom contacted 50 nm thick GST line cells used in the experiments were fabricated on 700 nm  silicon dioxide ($SiO_2$) thermally grown on Silicon wafers as described in  \cite{DirisaglikBakanJuradoEtAl2015}. Devices with varying widths and lengths were fabricated using 90 nm technology. Design widths start from 40 nm, well below the expected capability of  lithography, and increase with 2 nm increments. We observe that at small device lengths the wider contact regions merge, hence GST structure is continuous from one contact region to the other, even for 40 nm design widths, while the narrow devices do not survive the pattern transfer process at longer design lengths. Hence, connectivity between the two contacts of a device is random for the cells that are long enough and the widths are at the lithography limit, e.g. cells with $L_{design} = 460 nm$, $W_{design} = 52 nm$ display 40\%-60\% probability of having electrical connectivity measured in 10 dies\footnote{10 dies from a single 200 mm wafer were used to demonstrate the proof of concept.} (Figure~\ref{fig:litho_width}). 
%%COMMENT
%\marten{@Ali, Helena: check footnote}

Cells within this range can be used as bits in a string specific to the device, with a functional and broken cell representing 1 and 0 respectively. That way each chip will have a secret key of its own, thereby forming a physical obfuscated key. The output from the proposed POK is reliable since the connectivity of the line cells does not change under normal circumstances (0-90$^{\circ}$C) \cite{WongRaouxKimEtAl2010}. A bias (yield lower or higher than 50\%) can be removed through simple privacy amplification methods as discussed in Section \ref{subsec:relibility_enhancement} to produce independent and identically distributed bits. 

Annealing the line cells to high temperature will cause void formation at unpredictable regions which may affect cell connectivity; hence adds another degree of randomness. Figure \ref{fig:sem_cell}(c) shows such a case where the void at the center may break the connectivity while the cell looks connected on the surface. 

The cell to cell variations at lithography limit are highly dependent on tools and process parameters; hence, the proposed device is immune to cloning. Also, GST is a soft material compared to silicon, $SiO_2$, $Si_3N_4$ and tends to erode very quickly under focused ion beam. This increases the time, effort and tool complexity required to tamper with the IC. With today's technology the manufacturer cannot choose his own key or find out what key was chosen by the lithography process. 


%Future efforts will include use of intermediate resistance states between amorphous and crystalline states to store bits, resulting in increased key density. 

==> Draft_eprint - Copy/sections/pcm.tex <==
\section{PCM-based POK}
\label{sec:pcm} 

\begin{figure}[!tb]
\centering
\includegraphics[width = 0.8\columnwidth]{./figs/ThreeContactSnapshots.pdf}
\caption{{ (a) Polycrystalline GST (rainbow) with three metal contacts (dark gray) and electrically insulating oxide (light gray). (b) Current flows nearly symmetrically from the top contact to the two bottom contacts. (c) When melting begins near one of the bottom contacts, the path to that contact becomes very conductive and the contact draws more of the current. Higher current densities melt more of the path, creating a feedback loop (thermal runaway). (d) A highly resistive amorphous plug blocks the left contact when the current ceases. The initial device-specific grain map determines which contact is plugged, and subsequent read pulses reveal a large resistance contrast between the two paths regardless of drift. (e) Transient current into both contacts.}}
\label{fig:ThreeContactSnapshots}
\end{figure}

GST is considered a nucleation dominated material because over typical crystallization temperatures the amorphous to crystalline transition is primarily driven by new crystal grains nucleating rather than templated growth at existing crystalline/amorphous interfaces. The grain boundary resistivity is higher and displays higher temperature sensitivity than crystalline grain resistivity. The location of grain boundaries depends on stochastic nucleation events and temperature dependent growth velocities during the fabrication process; hence, there is intrinsic device-to-device variability in grain maps. We propose a device that produces a random bit dependent on an initial device specific grain map.  It is not possible to detect grain boundaries or amorphized regions using scanning electron microscopy. This makes a POK using this approach difficult to read with a physical attack. Transmission electron microscopy is capable of such differentiation, but requires time intensive and costly techniques (creating nm scale cross sections and physically moving them into the path of an electron beam), making it difficult to read a large number of bits this way.




%GST is considered a nucleation dominated material because over typical crystallization temperatures the amorphous to crystalline transition is primarily driven by new crystal grains nucleating rather than templated growth at existing crystalline/amorphous interfaces. The grain boundary resistivity is higher and displays higher temperature sensitivity than crystalline grain resistivity. The location of grain boundaries depends on stochastic nucleation events and temperature dependent growth velocities during the fabrication process; hence, there is intrinsic device-to-device variability in grain maps. We propose a device that produces a random bit dependent on an initial device specific grain map. Physically, the bit takes the form of an amorphous plug near one of two contacts (the two bottom contacts in Figure~\ref{fig:ThreeContactSnapshots}). It is not possible to differentiate amorphous material from crystalline material or detect grain boundaries using scanning electron microscopy. This makes a POK using this approach difficult to read with a physical attack. Transmission electron microscopy is capable of such differentiation, but requires time intensive and costly techniques (creating nm scale cross sections and physically moving them into the path of an electron beam), making it difficult to read a large number of bits this way.

Phase change materials typically have negative temperature coefficients of resistivity (TCR) which gives rise to thermal runaway when a sufficiently large voltage pulse is applied. Hence, if there are two competing current paths, one melts and amorphizes while the other does not experience current densities sufficient for melt and remains unchanged. Thermal runaway is determined by asymmetry in the initial grain map (Figure~\ref{fig:ThreeContactSnapshots}a). We demonstrate this concept through PCM device simulations using a finite-element phase change material model~\cite{Dirisaglik2014, Faraclas2014, Faraclas2011} which tracks temperature dependent nucleation, growth, and amorphization in GST (Figure~\ref{fig:ThreeContactSnapshots}). Temperature, phase, and electric-field dependent material parameters for crystalline GST, amorphous GST, and grain boundaries are extracted from experimental measurements~\cite{Adnane2012, Adnane2015, DirisaglikBakanJuradoEtAl2015}. Imperfections in fabrication processes can cause conductivity biases not related to the grain map and should be accounted for in process design.

The high resistivity contrast between amorphous and crystalline states is not affected by small ($\thicksim$ 0.1V) read pulses and crystallization of the amorphous state takes >10 years at 85$^{\circ}$C, making our proposed POK very reliable \cite{WongRaouxKimEtAl2010}.





==> Draft_eprint - Copy/sections/related_works.tex <==
\section{Background and Related Work}
\label{sec:notation_background}

In this section, we provide background and related work on reliability enhancement techniques, lithography-based PUFs and PCM-based PUFs. 

\subsection{Reliability enhancement techniques}
\label{subsec:relibility_enhancement}

%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/RepFE.pdf}
%\caption{Reproduction Procedure of Fuzzy Extractors~\cite{dodis2004fuzzy}}
%\label{fig:RepFE}
%\end{figure}  


%To generate a random secret key  from a noisy source, two problems must be solved: Reliability and De-correlation of source bits. % of raw output bits. 

%\vspace{3mm}

%\noindent
%\textbf{Reliability:} 
%Since the raw output from a noisy source is intrinsically noisy, we develop some approaches to produce a reliable raw output. 
%Without loss of generality, we consider a POK with only single pair of challenge and response $\vect{(c,r)}$.
In general, there are two approaches to make a POK reliable: Response Reinforcement and  Error Correction.

%\marten{Do we mention somewhere the other approaches based on ECC such as syndrome decoding by Mandel Yu and the use of pointers ... I think Ben wrote some of this in the FE paper we are working on?}

\vspace{3mm}

\noindent
\textbf{Response Reinforcement:} Response reinforcement  upgrades a PUF's reliability by using normal detrimental IC aging effects. Bhargava et al. \cite{BhargavaMai2013} demonstrate a one-time post-manufacture step of hot carrier injection stress in one of the NMOS transistors in a sense amplifier. The enhanced offset magnitude of the sense amplifier for both positive and negative polarities eliminates chances of errors due to environmental (voltage and temperature) variations and aging. Additional error correction circuit overhead and possible  information leakage  through helper data, see below, are alleviated in this approach. Even though 1.7 years of reliable operation is simulated by bake experiment, the deleterious long stress time of 125s for a feature size of 65 nm might affect reliability at matured stages. ~

\begin{figure}[!t]
\centering
\includegraphics[width = 0.6\columnwidth]{figs/FullPOKFEPR02.pdf}
\caption{A Digital PUF based on a POK architecture where POK represents the basic POK enhanced with a Fuzzy Extractor (FE) in Rep mode (using a RECovery procedure and Privacy Amplification or PA)  and extended with a Pseudo Random Function (PRF). 
%
%, FE, NVM, TRNG, SS, PA, PR, $h,s,W,W',k$ denote Physical Obfuscated Keys, Fuzzy Extractor, Non-Volatile Memory, True Random Number Generator, Secure Sketch, Privacy Amplification, PseudoRandom Functions, helper data, random string, a raw output of PK, noisy version of W and random key, respectively 
%%COMMENT
%\marten{@Ha: Can you use PRF instead of PR. Can you remove the TRNG/NVM: we just need a hard coded $s$ -- you can draw a NVM box.}
} 
\vspace{-1 em}
\label{fig:DigitalPUF}
\end{figure}


%\marten{Text right hand side Figure 1 is too small and should also be  aligned, e.g. left aligned or all colons are aligned. Here POK refers to a ``basic'' POK which is enhanced to a full POK architecure. Replace SS by Dec (notice SS is only used during the generation of the helper data, it does not provide decoding functionality right? And if SS has multiple modes of operation, then this should be clearly indicated in the text and figure.}

\vspace{3mm}

\noindent
\textbf{Error Correction:} Compared to response reinforcement,  error correction does not change the behavior of the output permanently. An extra circuit implements an error correction algorithm. Several constructions have been proposed: Fuzzy Extractors (FEs)~\cite{dodis2004fuzzy}, Computational Fuzzy Extractors~\cite{FullerMengReyzin2013}, and LPN-based PUFs~\cite{HerderRenDijkEtAl2016}. We notice that there are many different ECC-based constructions as shown in~\cite{Delvaux2014,Nguyen2015}. 
 Without loss of generality in terms of our discussion regarding hardware overhead and efficiency, we focus on FE~\cite{dodis2004fuzzy}. 

FE has two procedures: $\mathrm{Gen}$ and $\mathrm{Rep}$, the latter depicted in Figure~\ref{fig:DigitalPUF}. $\mathrm{Gen}$ takes basic POK output $W$  and a true random string $s$ as inputs and produces output $(h,s)$ where $h$ represents helper data. % and $k$ is a reliable and random secret key.
%; the  POK architectur $(h,s)$ represents a challenge from which 
  Helper data $h$ and random string $s$ are programmed in the POK architecture and used to reconstruct $W$ and a derived key $k$ from a noisy version $W'$ generated as a result of a next measurement of the noisy source in the Rep procedure. $\mathrm{Gen}$ generates helper data (i.e., parity check information) $h$ for $W$ using an error-correcting code in, what is called, a \textit{Secure Sketch} (SS). SS uses a random bit vector $x$ for this purpose, i.e., $h\leftarrow \mathrm{SS}(W,x)$. %In a nutshell, $(h,s)\leftarrow \mathrm{Gen}(x,s,W)$. 





%\ha{@Marten: the way i introduce the role of SS and PA is fine to you?}

Figure~\ref{fig:DigitalPUF} depicts the Rep procedure of a FE~\cite{dodis2004fuzzy} in a POK architecture.
Rep takes as input a next measurement $W'$ of basic POK output. $W'$ is a noisy version of $W$. If $W'$ and $W$ are different in $\leq d$ positions (i.e., the Hamming distance $d_{\mathrm{H}}(W',W)\leq d$), then the helper data $h$ from the Gen procedure allows a Recovery  procedure (REC) to reconstruct $W$ from $W'$. In fact, REC can be thought of as the reverse algorithm of SS. 
Next a random key $k$ is generated by applying a de-correlation process, called \textit{Privacy Amplification} ($\mathrm{PA}$),  to $W$. This is needed because the POK may produce correlated bits, but more important, within the attacker's view the helper data $h$ (and random string $s$) can easily be read because $h$ (and $s$) is either stored in NVM or hard coded by fuses, and this means $h$ is known to the adversary and conditioned on $h$ the reconstructed bits in $W$ are correlated. PA computes  $k \leftarrow \mathrm{PA}(W,s)$ and involves a hash function~\cite{dodis2004fuzzy}.  Since $W$ is reliably reconstructed, $k$ is also reliably reconstructed  and due to PA, $k$ is a random secret key. In Figure~\ref{fig:DigitalPUF}  $k$ is used for a digital PUF which if taking a challenge $c$ as input, produces an output response $r=\mathrm{PRF}_k(c)$ where PRF is a pseudo random function.
 % the bits in $W$ are correlated through the helper data $h$, which if stored in NVM or if hard coded by fuses can easily be read by an adversary.

%To generate a random key $k$ from correlated bits of $W$ (de-correlation process), a process called \textit{Privacy Amplification} ($\mathrm{PA}$) is required, i.e.,  $k \leftarrow \mathrm{PA}(W,s)$ which involves a hash function as shown in~\cite{dodis2004fuzzy}. 



%with the condition $d_{\mathrm{H}}(W',W)\leq d$. 
%Thus, $W \leftarrow \mathrm{SS}(W',h)$ and then
%Next the secret key $k$ is reproduced as $k \leftarrow \mathrm{PA}(W,s)$. Figure~\ref{fig:DigitalPUF} depicts the Rep procedure of a FE~\cite{dodis2004fuzzy} in a POK architecture. In a nutshell, $k \leftarrow \mathrm{Rep}(s,h,W')$.



%Compared to a FE, the constructions in~\cite{FullerMengReyzin2013,HerderRenDijkEtAl2016} also have Gen and Rep, but they can correct a larger number of errors if the measurement noise is \textit{independent and identically distributions} (i.i.d). Moreover, there are also many different ECC-based constructions as shown in~\cite{Delvaux2014,Nguyen2015}. 



Error correction based approaches have the following limitations:

\begin{itemize}
%\item \textit{Reliability.} 
% If the noise is large enough to violate condition $d_{\mathrm{H}}(W',W)\leq d$, then the reliability of FEs is also not guaranteed. 
 
  % (2) In~\cite{Delvaux2014,Nguyen2015} it is shown that the existence of helper data $h$ can leak information about the secret key $k$, i.e., the attacks by manipulating the helper data of POK allow the adversary determine $k$ ~\cite{Delvaux2014} or the adversary can directly use the helper data to get $k$ without manipulating $h$~\cite{Nguyen2015}. 
%(For completeness, since the constructions in ~\cite{FullerMengReyzin2013,HerderRenDijkEtAl2016} are based on Learning Parity with Noise (LPN), their security only needs to assume i.i.d. measurement noise or some other conjecture concerning measurement noise.) 
%It is also required to know at least \textit{min-entropy} of $W$ for measuring the security of $k$ and thus, the same problem persists for FE. More important,
% In~\cite{Delvaux2014,Nguyen2015} it is shown that the existence of helper data $h$ can leak the information about the secret key $k$.
% or the raw output of POK. 

\item \textit{Hardware Overhead.} As pictured in Figure~\ref{fig:DigitalPUF}, besides the basic POK circuit, several additional digital circuits (depicted in grey) need to be implemented and this accounts for a large hardware overhead of the final POK architecture. 
%Also PA needs a sufficient number of source bits in $W$ as input and this means that the POK must 


%described in ~\cite{dodis2004fuzzy,FullerMengReyzin2013,HerderRenDijkEtAl2016,Delvaux2014,Nguyen2015}, all ECC-based constructions require additional hardware circuitry such as a True Random Number Generator, Error Correction Encoder/Decoder (in Secure Sketch), and Hash Function (in Privacy Amplification). Thus, besides the basic POK circuit, the need to implement several additional digital circuitry makes for a significantly larger hardware overhead for the final POK architecture. 

\item \textit{Efficiency.} Since many digital processes are involved in producing a secret key $k$, the efficiency of POK-based systems is  significantly reduced in terms of execution time and power consumption (see~\cite{BhargavaCakirMai2012,BhargavaMai2013}). 
%\ha{@Marten: I think we should not introduce any number here because we cannot make complete design to do any comparison.}
%In~\cite{BhargavaCakirMai2012,BhargavaMai2013}, it is pointed out that most ECC implementations require $>2000$ cycles and $>3000$ SRAM bits to generate a reliable 128-bit key $k$. 

\end{itemize}

The limitations discussed above can be avoided if the basic POK output bits are intrinsically reliable: All the grey-color blocks in Figure~\ref{fig:DigitalPUF} can be removed. \textit{Response reinforcement}  can also avoid these limitations but it is only applicable to bi-stable memory and requires an additional process per POK.

\vspace{3mm}

\noindent
\textbf{De-correlation.} Even if we have an intrinsically reliable basic POK, its  output bits are likely correlated. Thus, we cannot directly use these bits as a secret key. We first need to de-correlate these bits by a privacy amplification process as described in the error correction based approach above. If PA is required, then the hardware overhead of the system is increased and the efficiency of system is reduced.   
However,
if the to-be-decorrelated bits are reliable and in addition have high min-entropy, a very simple trick used in the construction of True Random Number Generators applies: We can perform an XOR operation on several correlated bits together to produce a response bit. This results in close to independent and identically distributed response bits. 
%%COMMENT
%\marten{need reference regarding this TRNG construction with XOR}

%\ha{Prof Marten: Why in FEs, we need PA instead of XOR trick? The input $W$ is reliable, and we can apply the XOR trick to the $W$. I am confused now at this point. It seems that something goes wrong here?????}

 
%To apply the output generated from a noisy random resource (for example POKs or PUFs) in secure systems, many types of error correction codes (ECCs) are proposed. Typically, the reliable and random bit string are required in secure systems and to do it, an extra information is produced based on the original output (a.k.a golden response) and it is called as \textit{helper data}. For the reproduction process, the output is measured again and it is usually noisy (i.e., has some mismatches with the golden response). This noisy output is combined with helper data to reconstruct the golden response by apply some ECC algorithms~\cite{Delvaux2014,Nguyen2015}. Actually, the existence of the helper data does not guarantee that the reproduction can be successfully done. All ECCs has a threshold for the number of errors presenting in noisy output. Moreover, the existence of helper data also hurts the security, hardware overhead and efficiency of the systems~\cite{Delvaux2014,Nguyen2015}. 
%
%Moreover, using ECCs only helps us to solve the reliability question, not the de-correlation problem if the noisy outputs are correlated. Thus, as shown in~\cite{dodis2004fuzzy}, the privacy amplification process is in need. Typically, the noisy output is collaborated with a short true random bit string (generated from a True Random Number Generator) and they are the input of a hash function. The output of hash function is provably random, i.e., not correlated or \textit{i.i.d.}. It is evident that this process significantly increases the hardware overhead reduces the efficiency of the system. 









\subsection{Lithography based PUFs}
\label{subsec:lithoPUF}

%\cite{SreedharKundu2011,KumarBurleson2013,KumarDhanuskodiKundu2014} Lithograpy based PUFs

Using optical lithography, devices and interconnect layers are printed layer by layer in specified patterns on semiconductor wafers using a monochromatic light source focused through a lens and mask system. The entire IC fabrication process consists of hundreds of patterning, deposition, etching, doping, and polishing steps, all with inherent variabilities~\cite{Mack2007,KunduSreedharSanyal2007,KumarDhanuskodiKundu2014,SreedharKundu2011}. These include irregularities in etching, doping and polishing steps, light source intensity fluctuations, lens and mask defects and alignment, defocus, and interference problems~\cite{KumarDhanuskodiKundu2014}. The variations in the final dimensions of a device are a combination of variations introduced by the lithographic exposure, photo-resist processing and etching steps. For typical logic and memory applications, these variations must be within tolerances required for the desired yield and reliability. For other applications however, such as security, these variations may be utilized to achieve inherent, true physical randomness. Process variations can be systematic, such as mask defects or deviations from layout design, which are reflected similarly on all dies, or ``random'', such as local fluctuations in exposure, etch, deposition or polishing steps, which result in device-to-device variations within each die or die-to-die variation.

%Current sub-wavelength lithographic techniques including phase-shift and interference techniques, enable printing of $\approx 10$ nm features  using a much longer wavelength UV light source (193 nm)~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}. 
%Due to the proximity effects, constructive or destructive interference from the slits of the mask result in wider or narrower printed lines~\cite{SreedharKundu2011}. The width variations can be significant enough to turn out zero line width or an open device in some of the destructive interference incidences with closely spaced pitches (defined as forbidden pitches)~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}. 
Several resolution enhancement techniques, such as optical proximity correction, alternating phase shift mask, and immersion lithography, which are used to overcome sub-wavelength lithographic challenges to print  $\approx 10$ nm features  using a much longer wavelength UV light source (193 nm)~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}, are intentionally avoided to engineer highly sensitive lithographic variations based PUFs (litho-PUFs)~\cite{KumarDhanuskodiKundu2014,SreedharKundu2011}. Exploiting linewidth, length, and height variations in lithography simulation of litho-PUFs with forbidden pitch, Sreedhar et al. demonstrated output voltage fluctuations as a function of focus variation in the simulated devices~\cite{SreedharKundu2011}. Kumar et al. addressed fluctuations in the light intensity and durations and focus variations due to wafer tilt and resist thickness variations and showed improved inter-die and inter-wafer uniqueness with lithography simulation in the forbidden pitch zone~\cite{KumarDhanuskodiKundu2014}. To improve the performance of litho-PUFs the systematic variations should be suppressed and the random variations preserved or enhanced \cite{KumarDhanuskodiKundu2014}. Forte et al. delineated OPC optimized for litho-PUF which enhances the random variations while reducing the systemic variations \cite{Forte2012a,Forte2012}.


Wang et al. proposed a stability guaranteed PUF based on random assembly errors which result in random permanent connections during a directed self assembly (DSA) process \cite{Puneet}. However, the results presented in \cite{Puneet} were obtained from simulations and did not contain hardware implementation data. The proposed PUF is also susceptible to invasive attacks.


%Two types of variations are observed in the device properties, random and systematic. For improving the performance of litho-PUFs, the systematic variations are suppressed while keeping the random variations unaffected~\cite{KumarDhanuskodiKundu2014}. Forte et al. delineated OPC optimized for litho-PUF which enhances the random variations while reducing the systemic variations~

%\subsection{Introduction of PCMs}
%
%To construct the Phase Change Memory storing the digital information, two different electrical resistivity of two alternative structural phases of a suitable material are exploited~\cite{ZhangKongChangEtAl2014}. Typically, PCM cell consists of a storage device and access device. The storage device is made in the way such that it can be programmed to either a low-resistivity \textit{crystalline phase} ($R \approx 10^2 \Omega$) or high-resistivity \textit{amorphous phase} ($R \approx 10^6 \Omega$) to represent the SET (logic-1) and the RESET (logic-0) state, respectively (see~\cite[Fig. 2]{ZhangKongChangEtAl2014}). To change the state from SET to RESET, a high magnitude and fast fall time pulse is applied to the storage device. Conversely, to change from RESET to the SET state, either a pulse with moderate magnitude and long duration is required. 

\subsection{PCM-based PUFs}

%In~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, Zhang \textit{et.al} described proposed a PUF design based on PCM. At the same setup condition, the resistance of each PCM is randomly defined due to the process variation. Hence, by comparing the resistances of two different PCM cells, one random bit can be produced. However, if the environmental conditions change, then the resistance of PCM cell also changes. Thus, the proposed PCM-based PUF is not reliable.

Phase change memory (PCM) is an emerging non-volatile computer memory technology \cite{WongRaouxKimEtAl2010}. It offers high speed, high endurance, and non-volatility. A typical PCM cell consists of a phase change material (typically $Ge_2Sb_2Te_5$ or GST) between two electrodes. A small volume of this material in between the two contacts can be changed quickly and reversibly between the amorphous phases and the crystalline phase - leading to a high resistance state (Reset) and low resistance state (Set) - by suitable electrical pulses that result in different self-heating. Amorphization is achieved by melting followed by abrupt cooling (melt-quench) whereas crystallization is achieved by maintaining the element above crystallization temperature for a sufficiently long period of time, either by a longer, lower voltage pulse or by a melting pulse followed by a longer fall time. The read operation is performed with a small voltage pulse such as not to disturb the crystalline state of the cell~\cite{WongRaouxKimEtAl2010,burr2010phase}. 
The process variations and programming sensitivity of PCM devices have been utilized by Zhang et al. for reconfigurable PUF , that dynamically generates updatable cryptographic keys. The address of two selected PCM cells is used as the challenge and the resistance comparison between the two cells is the response~\cite{ZhangKongChangEtAl2014}. 

%changes back and forth to high (amorphous, $R_{high}$) and low (crystalline, $R_{low}$) resistance states when different electrical pulses are applied across the electrodes. The reversible transitions between these two states are called set ($R_{high}$ to $R_{low}$) and reset ($R_{low}$ to $R_{high}$). 


%\subsection{Resistance drift and decay of PCMs}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/resistance_drift.png}
%\caption{Resistance Drift and Decay of PCMs.}
%\label{fig:Drift_Decay_PCM}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/resistance_drift_00.png}
%\caption{Resistance Drift and Decay of PCMs with different initial condition of RESET.}
%\label{fig:Drift_Decay_PCM_00}
%\end{figure}
%
%In order to build TLP based on PCM, the basic phenomena of PCM is exploited, i.e., the phenomena \textit{resistance drift and decay of PCM} as depicted in ~\cref{fig:Drift_Decay_PCM}. After the RESET with a certain initial condition (i.e., voltage and temparature), the resistance of PCM cell increases in the duration $[t_0,t_1]$ (the drift phase) and then it decreases after the saturation point $t_1$ (the decay phase). In~\cref{fig:Drift_Decay_PCM_00}, it is evident that the \textit{drift and decay} curve heavily depends on the initial condition of the RESET. Moreover, even if all the PCM cells are initialized under the same condition of the RESET, they have different curves of drift and decay. 




==> Draft_eprint - Copy/sections/related_works_old.tex <==
\section{Background and Related Work}
\label{sec:notation_background}

In this section, we provide a background and related works, i.e., reliability enhancement techniques, lithography based PUFs and PCM-based PUFs. 

\subsection{Reliability enhancement techniques}
\label{subsec:relibility_enhancement}

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/RepFE.pdf}
\caption{Reproduction Procedure of Fuzzy Extractors~\cite{dodis2004fuzzy}}
\label{fig:RepFE}
\end{figure}  


In the PUF's literature, to generate a random secret key which can be used in secure systems from the noisy source, two following problems must be solved: 1) Reliability and 2) de-correlation of raw output bits. 

\textbf{Reliability.} Since the raw output from noisy source is intrinsically noisy, we develop some approaches to produce a reliable raw output. Without loss of generality, we consider a POK with only single pair of challenge and response $\vect{(c,r)}$. Typically, there are two approaches to make the $\vect{r}$ reliable: \textbf{response reinforcement} and \textbf{ECC-based approach}

\textit{Reinforcement approach.} \ha{Nafisa's writing. The bad things for this approaches is: additional process, manpower and technique efforts required, and not general, i.e., only applied to bi-stable memory based POKs} 


\textit{ECC-based approach.} Compared to response reinforcement, this approach does not change the behavior of output permanently after doing additional process. Instead, an extra circuit which implements the error correction algorithm is required and we have the several constructions, e.g., Fuzzy Extractors (FEs)~\cite{dodis2004fuzzy}, Computational Fuzzy Extractors~\cite{FullerMengReyzin2013}, LPN-based PUFs~\cite{HerderRenDijkEtAl2016}. Without loss of generality, we focus on FE~\cite{dodis2004fuzzy}. A FE contains two procedures: $\mathrm{Gen}$ and $\mathrm{Rep}$. $\mathrm{Gen}$ takes the noisy output $W$ and true random string $s$ as the input and produces the output as $(h,s,k)$ where $h$ is the called helper data and $k$ is the secret key which is reliable and all its bits are independent. Helper data $h$ is used to reconstruct $W$ from its noisy version $W'$ generated from noisy source in Rep procedure by using an algorithm \textit{Secure Sketch} (SS) with a random bit input $x$, i.e., $h\leftarrow \mathrm{SS}(W,x)$. To generate $k$, a process is called \textit{Privacy Amplification} ($\mathrm{PA}$) is required, i.e.,  $k \leftarrow \mathrm{PA}(W,s)$. As shown in~\cite{dodis2004fuzzy}, the hash function is involved in PA. In a nutshell, $(h,s,k)\leftarrow \mathrm{Gen}(s,W)$. 

In Reproduction procedure (Rep), the raw POK output $W'$ is measured and it is a noisy version of $W$, i.e., $W'$ and $W$ are different in maximum $d$ positions or $d_{\mathrm{H}}(W',W)\leq d$. Typically, the helper data $h$ in Gen procedure is generated in a way such that the secure sketch SS can reconstruct $W$ from $W'$ with the condition $d_{\mathrm{H}}(W',W)\leq d$. Thus, $W \leftarrow \mathrm{SS}(W',h)$ and then the secret key $k$ is reproduced as $k \leftarrow \mathrm{PA}(W,s)$. Figure~\ref{fig:RepFE} depicts the Rep produce of FEs in~\cite{dodis2004fuzzy}. Compared to FEs, two constructions in~\cite{FullerMengReyzin2013,HerderRenDijkEtAl2016} also have two Gen and Rep, but they can correct more number of errors if the measurement noise in raw output follows \textit{independent and identically distributions} (i.i.d). Moreover, we can have many different types of ECC-based as shown in~\cite{Delvaux2014,Nguyen2015}. 

However, all the ECC-based approaches have the following problems.

\begin{itemize}
\item \textit{Security.} In FE construction~\cite{dodis2004fuzzy}, the security of $k$ is provided if the \textit{min-entropy} of raw output $W$ is known. However, this is \textit{impossible} mission in practice due to the large number of POK's output bits and all the bits are correlated. In other words, we cannot exactly address the security of POK-based system in the context of FEs. Moreover, the if the noise is big enough to make the condition $d_{\mathrm{H}}(W',W)\leq d$ does not hold, then security of FEs is also not guaranteed. In~\cite{FullerMengReyzin2013,HerderRenDijkEtAl2016}, since the two constructions are based on Learning Parity with Noise (LPN), the security is only provided when the measurement noise is \textit{i.i.d} which does not hold in practice. Moreover, we also need to know at least \textit{min-entropy} of $W$ for measuring the security of $k$ and thus, they also face the same problem for FE. More important, in~\cite{Delvaux2014,Nguyen2015}, it is shown that the existence of helper data $h$ can leak the information of the secret key $k$/ the raw output of POK $W$ or the adversary can fully retrieve the secret key/ the raw output $W$. 

\item \textit{Hardware Overhead.} As described in~\cite{dodis2004fuzzy,FullerMengReyzin2013,HerderRenDijkEtAl2016,Delvaux2014,Nguyen2015}, all ECC-based constructions require additional hardware circuitry such as True Random Number Generation, Error Correction Code algorithm (in Secure Sketch), Hash Functions (in Privacy Amplification), etc. Thus, beside the POK circuit, we need to implement several additional digital circuitry which makes the final hardware overhead is big. 

\item \textit{Efficiency.} Since many digital processes are involved in producing a secret key $k$, the efficiency of POK-based system significantly reduces in terms of execution time, power consumption. In~\cite{BhargavaCakirMai2012,BhargavaMai2013}, it is pointed that most ECC implementations $>2000$ cycles and $>3000$ SRAM bits to generate reliable 128-bit key $k$. 

\end{itemize}

From this analysis, we can see that all the problems mentioned above will be dropped if the raw outputs of POK is intrinsically reliable. Typically, \textit{response reinforcement} approach can solve all these problems but the shortcomings are: not general (i.e., only applied for bi-stable memory), manpower and technique efforts are in need and additional process is required.

\textbf{De-correlation.} As discussed above, all the raw output bits of POK (i.e., digital interpretation of analog output of POK) are correlated. Thus, we cannot directly use the raw output of POK as a secret key in secure systems. We need to de-correlate the raw output of POK by the privacy amplification process as described in ECC-based approaches if the raw output of POK is noisy. It is evident that, if PA is required, then the hardware overhead of system is increased and the efficiency of system is reduced.   

If the raw output is reliable (for example, after the response reinforcement), we can use a very simple trick in True Random Number construction, i.e., xoring several correlated bits together to produce a constructed bit. All constructed bits will be indepedent and identically distributed.  

\ha{Prof Marten: Why in FEs, we need PA instead of XOR trick? The input $W$ is reliable, and we can apply the XOR trick to the $W$. I am confused now at this point. It seems that something goes wrong here?????}

 
%To apply the output generated from a noisy random resource (for example POKs or PUFs) in secure systems, many types of error correction codes (ECCs) are proposed. Typically, the reliable and random bit string are required in secure systems and to do it, an extra information is produced based on the original output (a.k.a golden response) and it is called as \textit{helper data}. For the reproduction process, the output is measured again and it is usually noisy (i.e., has some mismatches with the golden response). This noisy output is combined with helper data to reconstruct the golden response by apply some ECC algorithms~\cite{Delvaux2014,Nguyen2015}. Actually, the existence of the helper data does not guarantee that the reproduction can be successfully done. All ECCs has a threshold for the number of errors presenting in noisy output. Moreover, the existence of helper data also hurts the security, hardware overhead and efficiency of the systems~\cite{Delvaux2014,Nguyen2015}. 
%
%Moreover, using ECCs only helps us to solve the reliability question, not the de-correlation problem if the noisy outputs are correlated. Thus, as shown in~\cite{dodis2004fuzzy}, the privacy amplification process is in need. Typically, the noisy output is collaborated with a short true random bit string (generated from a True Random Number Generator) and they are the input of a hash function. The output of hash function is provably random, i.e., not correlated or \textit{i.i.d.}. It is evident that this process significantly increases the hardware overhead reduces the efficiency of the system. 









\subsection{Lithography based PUFs}

%\cite{SreedharKundu2011,KumarBurleson2013,KumarDhanuskodiKundu2014} Lithograpy based PUFs

In optical lithography, devices and metal layers are printed in patterns on semiconductor wafers using a monochromatic light source which is focused through a lens system on a mask1. The entire IC fabrication process consists of several patterning, deposition, etching, doping, and polishing steps that comprise inherent variabilities and hence, prohibit precisely accurate reprint~\cite{Mack2007,KunduSreedharSanyal2007,KumarDhanuskodiKundu2014,SreedharKundu2011}. These variations in physical and electrical properties of the fabricated devices arise due to the aberrations in etching, doping and polishing steps, light source intensity imperfections, lens system and mask alignment issues, defocus, and interference problems~\cite{KumarDhanuskodiKundu2014}. 
Based on the everlasting consumer demands for smaller, faster, cheaper, and less energy hungry electronic devices, the expedition of the microelectronics industry has involved downsizing of the device feature size following Moore's Law for four decades~\cite{Moore1965}. However, the lack of improvements in the wavelength of the light source for past two decades led to the sub-wavelength lithographic approach where a larger wavelength of the light source (193 nm) is used for printing much narrower devices~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}. Due to the proximity effects, constructive or destructive interference from the slits of the mask result in wider or narrower printed lines~\cite{SreedharKundu2011}. The width variations can be significant enough to turn out zero line width or an open device in some of the destructive interference incidences with closely spaced pitches (defined as forbidden pitches)~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}. 
Even though several resolution enhancement techniques (such as optical proximity correction (OPC), alternating phase shift mask, and immersion lithography) are used to overcome these sub-wavelength lithographic challenges~\cite{KunduSreedharSanyal2007}, intentional avoidance of these schemes are also found in literature to engineer highly sensitive lithographic variations based PUFs (litho-PUFs)~\cite{KumarDhanuskodiKundu2014,SreedharKundu2011}. Exploiting linewidth, length, and height variations in lithography simulation of litho-PUFs with forbidden pitch, Sreedhar et al. demonstrated output voltage fluctuations as a function of focus variation in the simulated devices~\cite{SreedharKundu2011}. Kumar et al. addressed fluctuations in the light intensity and durations and focus variations due to wafer tilt and resist thickness variations and showed improved inter-die and inter-wafer uniqueness with lithography simulation in the forbidden pitch zone~\cite{KumarDhanuskodiKundu2014}.
Two types of variations are observed in the device properties, random and systematic. For improving the performance of litho-PUFs, the systematic variations are suppressed while keeping the random variations unaffected~\cite{KumarDhanuskodiKundu2014}. Forte et al. delineated OPC optimized for litho-PUF which enhances the random variations while reducing the systemic variations~\cite{Forte2012a,Forte2012}










%\subsection{Introduction of PCMs}
%
%To construct the Phase Change Memory storing the digital information, two different electrical resistivity of two alternative structural phases of a suitable material are exploited~\cite{ZhangKongChangEtAl2014}. Typically, PCM cell consists of a storage device and access device. The storage device is made in the way such that it can be programmed to either a low-resistivity \textit{crystalline phase} ($R \approx 10^2 \Omega$) or high-resistivity \textit{amorphous phase} ($R \approx 10^6 \Omega$) to represent the SET (logic-1) and the RESET (logic-0) state, respectively (see~\cite[Fig. 2]{ZhangKongChangEtAl2014}). To change the state from SET to RESET, a high magnitude and fast fall time pulse is applied to the storage device. Conversely, to change from RESET to the SET state, either a pulse with moderate magnitude and long duration is required. 

\subsection{PCM-based PUFs}

%In~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, Zhang \textit{et.al} described proposed a PUF design based on PCM. At the same setup condition, the resistance of each PCM is randomly defined due to the process variation. Hence, by comparing the resistances of two different PCM cells, one random bit can be produced. However, if the environmental conditions change, then the resistance of PCM cell also changes. Thus, the proposed PCM-based PUF is not reliable.

Phase change memory (PCM) is an emerging non-volatile computer memory technology. It offers high speed, high endurance, low power programming and good cell scalability. A typical PCM cell consists of a phase change material (typically $Ge_2Sb_2Te_5$ or GST) between two electrodes. A portion of this material changes back and forth to high (amorphous, Rhigh) and low (crystalline, Rlow) resistance states when different electrical pulses are applied across the electrodes. The reversible transitions between these two states are called set (Rhigh to Rlow) and reset (Rlow to Rhigh). The read operation is performed with a small voltage by not disturbing the state of the cell~\cite{WongRaouxKimEtAl2010,burr2010phase}. 
The process variations and programming sensitivity of PCM is utilized in reconfigurable PUF implementation by Zhang et al. where dynamically updatable cryptographic keys are generated. The address of two selected PCM cells is used as the challenge and the resistance comparison of the two cells is the response~\cite{ZhangKongChangEtAl2014}. 




%\subsection{Resistance drift and decay of PCMs}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/resistance_drift.png}
%\caption{Resistance Drift and Decay of PCMs.}
%\label{fig:Drift_Decay_PCM}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/resistance_drift_00.png}
%\caption{Resistance Drift and Decay of PCMs with different initial condition of RESET.}
%\label{fig:Drift_Decay_PCM_00}
%\end{figure}
%
%In order to build TLP based on PCM, the basic phenomena of PCM is exploited, i.e., the phenomena \textit{resistance drift and decay of PCM} as depicted in ~\cref{fig:Drift_Decay_PCM}. After the RESET with a certain initial condition (i.e., voltage and temparature), the resistance of PCM cell increases in the duration $[t_0,t_1]$ (the drift phase) and then it decreases after the saturation point $t_1$ (the decay phase). In~\cref{fig:Drift_Decay_PCM_00}, it is evident that the \textit{drift and decay} curve heavily depends on the initial condition of the RESET. Moreover, even if all the PCM cells are initialized under the same condition of the RESET, they have different curves of drift and decay. 




==> sections/acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:Acknowledgements}
The devices are fabricated at IBM T.J. Watson Research Center
and characterized at UConn, supported by the U. S. National
Science Foundation under awards \# ECCS 0925973 and ECCS
1150960. The characterization and analysis efforts of R.S.K., N.N. and J.S. and the problem statement and motivation of C.J. and H.P.N. are supported by 
%Multidisciplinary University Research Initiatives (MURI) Program. 
%This project was supported in part 
AFOSR MURI under award number FA9550-14-1-0351.
The authors would like to thank Dr Chung Lam, Dr Yu Zhu, Dr Simone Raoux, Dr Norma Sosa, Dr Matthew
BrightSky and Dr Adam Cywar for their contributions to device fabrication at IBM T.J. Watson Research Center.

==> sections/experiment.tex <==
\section{Experiment}
\label{sec:experiment}



==> sections/granularity.tex <==
\section{The Variability of Granularity of PCM}
\label{sec:granularity}



==> sections/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Since \textbf{Physical Unclonable Functions} (PUFs)~\cite{Pappu2001} were introduced in 2001, they have been considered as promising hardware security primitives for building secure systems such as IP protection, authentication protocol, cryptographic primitives, etc~\cite{Kumar2008,Armknecht2009,Maes2010,Yu2011,Brzuska2011}. 

PUFs exhibit a random challenge-response behavior, i.e., a random-looking response is generated by PUF when queried with a specific challenge based on intrinsic manufacturing variations. Since the PUFs is built based on the manufacturing process variation, all the PUF's behavior is unique and \textit{physically unclonable}.

In practice, we can partition all PUF designs into two different categories: \textit{strong PUF} and \textit{weak PUFs} (or Physically Obfuscated Keys - POKs)~\cite{Gassend2003a}. The major difference between those two categories is that the former has a large number of challenge-response pairs (CRPs), while the latter has a limited number of CRPs. In this paper, we focus on POKs. POKs can be used for IP protection, authentication protocol~\cite{Suh2007}, tamper-resistant storage of random keys or building digital PUFs~\cite{Gassend2003a} due to its important security properties such as physical unclonability, uniqueness, tamper-resistance, unpredictability (or randomness), etc. In this paper, we focus on the following important properties of POK for evaluating our proposed POK constructions:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device.

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/POK_DigitalPUF.pdf}
\caption{Architecture of a physically obfuscated PUF in~\cite{Gassend2003a}}
\label{fig:DigitalPUF}
\end{figure}

The first POK-based system was introduced as a \textit{digital PUFs}~\cite{Gassend2003a} where the secret key of the secure systems is the response of a fixed challenge (see Figure~\ref{fig:DigitalPUF}). Since there is no secret key stored in a non-volatile memory (NVM) in POK-based system, the adversary cannot directly retrieve the secret key from the device. 

Typically, the POK circuit consists of two parts: randomness source and randomness extraction circuit. The randomness extraction circuit extracts and converts the analog signal from randomness source into \textbf{the raw output (digital signal)} which can be used in digital systems. For example, in RO-based POK~\cite{Suh2007}, the randomness source is the delay randomness in each circuit component,  and randomness extraction circuit are Ring Oscillators (ROs), counter and comparator. A pair of ROs is chosen and their frequencies (measured by counter) are compared to each other to procedure one bit output. 

Moreover, since the raw POK's outputs are tamper-resistant, the security of system is enhanced in term of tamper-resistance. In other words, if the adversary physically opens the device for reverse engineering purpose, then the raw POK's outputs are changed. Hence, if the raw POK's outputs are used as a secret key in symmetric key system or as a key mask in public key systems, the adversary cannot physically open the device for retrieving the secrets.  

However, to be used in secure systems, the raw POK outputs and \textit{independent and identically distributed-i.i.d.} (i.e. not correlated). Both of those required properties are not satisfied for raw POK outputs. To over come the reliability problem, Error Correction Code (ECCs)~\cite{Gassend2002a,Suh2007} or Fuzzy Extractor~\cite{dodis2004fuzzy} is exploited to make PUF's output stable. However, we have to face with many challenges in terms of \textbf{security, hardware overhead and efficiency} when the ECC is applied to enhance the reliability of POK as discussed in detail in Section~\ref{subsec:relibility_enhancement}. 

 



%\marten{for what?}
%\marten{what has PUF to do with the abstract? may be say ``since PUF and as a special class POKs were''}
%There are many proposed PUF designs, for example Arbiter PUFs (APUFs)~\cite{Lim2004}, Controlled PUFs~\cite{Gassend2002a}, Ring Oscillator PUFs (RO PUFs), XOR PUFs~\cite{Suh2007}, Lightweight Secure PUFs~\cite{Majzoobi2008a}, Composite PUFs~\cite{Sahoo2014} and LPN-based PUFs~\cite{HerderRenDijkEtAl2016}, Phase Change Memory based
%PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, etc. 
%\marten{above line can go to related work}
%Typically, PUFs exhibit a random challenge-response behavior, i.e., a random-looking response is generated by PUF when queried with a specific challenge based on intrinsic manufacturing variations. Since the PUFs is built based on the manufacturing process variation, all the PUFs are different and  \textit{physically unclonable}. 
%\marten{typically? I think always.  Do you mean different PUFs from the same PUF design are all different? We only assume that manufacturing variations cannot be physically cloned.}
%Due to the physically unclonable property, there is a large number of proposed applications which either complement or substitute traditional cryptographic algorithms~\cite{Kumar2008,Armknecht2009,Maes2010,Yu2011,Brzuska2011}.
%\marten{algorithms such as? -- may want to focus on what POKs are good for}
% In practice, we can partition all PUF designs into two different categories: \textit{strong PUF} and \textit{weak PUFs} (or Physically Obfuscated Keys - POKs)~\cite{Gassend2003a}. The major difference between those two categories is that the former has a large number of challenge-response pairs (CRPs), while the latter has a limited number of CRPs. In this paper, we focus on POKs.
% \marten{see above - why are these interesting?} For the POK, there are many properties \marten{what are the others? -- need to know this how else can we claim we design new POKs} and here three most important properties of POK are:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device. \marten{PUF to POK?}




  
  
% However, the presence of ECC can reduce the security of PUFs, i.e., the adversary can develop some attacks on PUFs~\cite{Delvaux2014,Nguyen2015} due to the presence of \textit{helper data} which is required for error correction process. \marten{Explain this reduction in security: You need to first explain that PA needs to be added because of the public helper data and that a hash of the corrected and amplified output should serve as a key (in PUF design for re-usability). You can give the example of a RO POK with 25\% noise under extreme temperature variations. One needs many POK output bits to get secure bits out. The question is also how does the helper data affect security? If one publishes many helper data for many responses, then in the PUF domain one can possibly break the PUF -- this is unknown. For POKs though we have just one helper data. And also we do not need the re-usability as for PUFs. So security is not reduced as for PUFs. Try to add this understanding by comparing the POK and PUF.} Moreover, using ECC has to pay a high cost in terms of hardware overhead, implementation efficiency as pointed in~\cite{BhargavaMai2013}. As an important note, the ECC-based approach only works if certain conditions are satisfied (see Fuzzy Extractor~\cite{dodis2004fuzzy}). \marten{It is better to indicate that the ECC approach with PA combined us what is now called FE. Best is to mention this earlier upfront. } \marten{If this is an important note, then you should explain these certain conditions -- and why this is important ! It now reads like an empty statement.}

For PUF design based on bi-stable memories the reliability of the PUF output can be significantly improved by output reinforcement process as discussed in~\cite{BhargavaCakirMai2012,BhargavaMai2013}, for example Hot Carrier Injection technique. Typically, this process changes the PUF's circuit characteristic permanently and thus, the PUF's output can be highly reliable. To achieve this goal, a suitable setup is required (\textcolor{red}{Ha: Chenglu and Nafisa can you verify this claim?}) and it is not always available to the PUF designer. It is evident that reinforcement process increases the manpower and technology efforts for PUF design. In additional, compared to the ECC-based approach, the response reinforcement is not general, i.e., it is only available to bi-stable memories. 

% as shown in~\cite{BhargavaCakirMai2012,BhargavaMai2013}. \marten{You should write ``For PUF design based on bi-stable memeories the reliability of the PUF output can be significantly ...'' at the start of the paragraph and delete this sentence.}
%
%For the ECC-based approach, to solve the i.i.d. problem, \marten{What is the iid problem? It was not explained earlier? Is it a problem? It becomes a problem if one feels that for correlated noise one implicitly needs to assume a computational hardness assumption which states that the FE approach also is secure with respect to such noise in that the correlations can not be computationally exploited. A sentence like this can be part of an earlier paragraph were you explain realiability, FE, helper data etc.} the raw output of POK after the error correction process must go through a \textit{privacy amplification process} which requires \textbf{a true random bit string} (see Fuzzy Extractors~\cite{dodis2004fuzzy}). \marten{input string? As you can see a bunch of my comments and text spread out in these paragraphs can be re-organized in a better logical order.} Actually, we have the following major challenges for using FEs for de-correlating POK's outputs: \marten{Actually? You like to now enumerate the challenges because you have explained the whole reliability problem in sufficient detail.}
%\begin{enumerate}
%\item \textbf{Security.} Since it is required to quantify the min-entropy of the raw POK's output for computing the final output of FEs and this is a \textit{impossible} mission in practice due to the large number of POK's output bits and its correlation, we cannot exactly address the security of POK-based system in the presence of FEs. \marten{Suggestion: Use separate paragraph headings such as ``security'' so that the above comments/text clearly explain what is happening.}
%\item \textbf{Hardware overhead.} The hardware footprint is significantly increased due to the presence of true random bit string.
%\marten{This is out of the blue. You need to explain FE using a picture and give enough details to explain where the TRNG comes in and why.}
%\item \textbf{Efficiency.} The efficiency of the POK-based systems is significantly reduced due to the use of hash function in FEs.   \marten{Again what is going on? You mean the PA implemented by the hash function reduces the rate of amount of secret output bit per POK bit.}
%\end{enumerate}
%\marten{I think we need a separate (sub?)section on reliability with a bunch of the above clearly cristalized in that section. The intro just gives a brief heads up with the main conclusion of that section.}

We \textbf{observe} that if the raw POK's output is reliable, then the de-correlation problem  can be solved in the simple way by using the de-correlation technique from the construction of True Random Number Generation. Typically, if we XOR many correlated bits together, the constructed bit is not biased and the independence and identically distribution property between the constructed bits are enhanced. Hence, we can solve the long term open and fundamental problem in PUF's research topic with a lightweight XOR-based network. Thus, the main question is that \textit{can we have intrinsically reliable POK design?}. If possible, then all the problems related to the reliability enhancement technique will be dropped. In other words, our POK design includes a raw reliable POK output and XOR-based network. Since, the POK's outputs are i.i.d, then all systems which are based on this POK can be \textbf{provably secure}. Note that, \textit{provable security} is also an long-term fundamental problem in hardware security research topic (see Section~\ref{subsec:relibility_enhancement}).

\marten{This paragraph is the core motivation and should be stressed as such -- let's push the whole reliability discussion out to a next section ``Reliability Enhancement and Related Work''}

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/UNOPOK.pdf}
\caption{Difference between UNO and POK/PUF}
\label{fig:unopok}
\end{figure}

\textbf{Contributions.}
In this paper, our main contributions are as follows. First, we observe that the lithographic process can provide a good random source in case of nano-scale technology. Typically, the lithographic process can be used to create \textbf{Unique Object - UNO}~\cite{Ruhrmair2011}. In~\cite{Ruhrmair2011}, the UNO is described as  ``A Unique Object is a physical system that, upon measurement by an external apparatus, exhibits a small, fixed set of inimitable analog properties that are not similar to any other objects''. In rough words, UNO is different from POK in the way we measure the objects. For POK, we have to use the internal apparatus to not expose the output of POK and UNO's output is not kept as secret. As an important property, the output of UNO is reliable. Figure~\ref{fig:unopok} shows the difference between the notions UNO and POK/PUF.

%\marten{Let's explain this in a picture and put this definition upfront where POK/PUF is explained. Here we can refer to the picture again and explain where the two solutions fall. The picture also indicates the noise problem, i.e. UNO is generally perfectly reliable and POK/PUF not and we push this boundary.}

Typically, the wires (connections) in a chip can be randomly connected or disconnected if we force the lithographic process to work with very small scales. This property is called as \textbf{variability of lithographic process}. Hence, the connectivity of each such wire can be converted to a random bit. Hence, a secret key/ a key mask based on the connectivity of wires can be constructed in secure protocols. Moreover, this secret key / key mask can be generated in reliable way. 

%\marten{You mean random secret key -- may be we should use ``random mask'' which is used to XOR the actual secret key with, there sult stored in non-volatile memory -- see the digital PUF picture. By the way a digital PUF hardcodes a key as POK from which a PUF is derived. } 

Specifically, a set of wires constructed by lithographic process is UNO but if this set is hidden, then we have POK instead of UNO. We will show that, if the adversary physically access the set of wires in the chip, then the connectivity of wires is changed, i.e., we have a tamper-resistant and reliable POK design. Since the width of wires is pretty small, we can have many random bits in a significantly small hardware footprint. \footnote{Needs to be checked by Ali/Helena etc.}

%\marten{Confusing. I thought it is about the external measurement apparatus. We can say that our solution is like a UNO in that it is noise-free.} 

In the PUF's literature, the lithographic process has been introduced to construct PUF designs as shown in~\cite{SreedharKundu2011,KumarBurleson2013,KumarDhanuskodiKundu2014}. However, the design philosophy of PUF designs in those papers is different (i.e., not use the connectivity of the wires) and the PUF's outputs are not reliable.  
%\marten{Either to related work, or consistently add such a paragraph for our second PCM solution.}

%However, if the adversary can physically access the device to observe the connectivity of wires, then the security of this random string is not guaranteed anymore. 

As a second contribution, we propose a novel Phase Change Memory (PCM) based POK. In the existing PCM-based PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, the resistances of two PCM cells, which are randomly defined by the process variation, are compared to produce a output bit. Due to the fluctuation in the current, the resistances can be changed and thus, the output is not reliable. Our proposed PCM-based POK is different from that in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} in terms of design philosophy, i.e., we use only one PCM cell to produce one bit output based on \textbf{the variability of granularity of PCM cells}. Our proposed PCM cell is randomly programmed as a ``left'' or ``right'' gate through which reliably a 0 or 1 is encoded. Thus, we can achieve a reliable PCM-based POK without using any reliability-enhancement techniques as mentioned above.  

To support all proposed theoretical results, we demonstrate the simulations and experiments in detail. 

% Compared to the method based on lithographic process, since no-one can physically observe the granularity inside the PCM cell, the proposed PCM-based POK is secure against physical attacks. 

The rest of paper is organized as follows. We discuss related work in Section~\ref{sec:notation_background}. Section~\ref{sec:lithography} presents the lithography based POK. The PCM-based POK is described in Section~\ref{sec:granularity}. Section~\ref{sec:experiment} demonstrates the simulated results on lithography and PCM based POKs. Section~\ref{sec:conclusion} concludes this paper. 
 



%In addition, the helper data is required and it is stored off-chip in non-volatile memories which is later used for correcting the errors in PUF's raw outputs.


 

%UNO~\cite{Ruhrmair2011}
%
%Digital PUF was first introduced in~\cite{Gassend2003a}
%
%In~\cite{Tuyls2006}, Tuyls et al. proposed a PUF design which has a single pair of challenge-response. 
%Actually, the response is used as cryptographic key and any attempts to breach the device will destroy the key. 
%This kind of system provides read-proof key storage, and is called as a weak PUF~\cite{Guajardo2007,Ruhrmair2009a} or 
%physically obfuscated key (POK)~\cite{Gassend2003}. A strong PUF has many CRPs and the adversary may access a set of CRPs but cannot sample exhaustively. However, POK has few CRPs and thus, as the security requirement, the CRPs must remain secret from the adversary. 
%
%For the POK, there are many properties and here three most important properties of POK are:  1) \textbf{Robustness:} the outputs are stable, 2) \textbf{Unpredictability:} the outputs are not predicted, i.e., should be randomly generated, 3)\textbf{Uniqueness:} the outputs are different from device to device
%
%% \textcolor{red}{Ha: how we can measure the uniqueness of proposed PCM-based POK?}.  
%
%One of the major research topics in PUFs is achieving a highly reliable PUF's responses or outputs. Since PUFs implementation is based on intrinsic manufacturing variations, the PUF behavior may be slightly different each time when the environmental conditions (e.g, temperature, supplying voltage) change~\cite{Lim2004}. To cope this problem, Error Correction Code (ECC)~\cite{Gassend2002a,Suh2007} or Fuzzy Extractor~\cite{dodis2004fuzzy} is exploited to make PUF's output stable. However, the presence of ECC can reduce the security of PUFs, i.e., the adversary can develop some attacks on PUFs~\cite{Delvaux2014,Nguyen2015}. Moreover, using ECC has to pay a high cost in terms of hardware overhead, implementation efficiency as pointed in~\cite{BhargavaMai2013}. In addition, the helper data is required and it is stored off-chip in non-volatile memories which is later used for correcting the errors in PUF's raw outputs. 
%
%As an alternative approach, the reliability of PUF's output can be significantly improved by reinforcement process as discussed in~\cite{BhargavaCakirMai2012,BhargavaMai2013}. Typically, this process will permanently change the PUF's circuit characteristic and thus, the PUF's output can be highly reliable. To achieve this goal, the special instrument is required (Chenglu can you verify this claim?) and it is not always available for the PUF designer.
%
%In recent years, it is shown that Phase Change Memories (PCMs) can be used to construct PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}. PCM is a nanoscale non-volatile memory and it has a good aging-resistance property. However, the output of PCM-based PUFs is not reliable as shown in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}. 
%Thus, if PCM is used to construct POK, then ECC or reinforcement process are in need. 
%
%In this paper, our main constructions are as follows. First, we observe that the lithographic process can provide a good random source in case of nano-scale technology. Typically, the wires (connections) in the devices can be randomly connected or disconnected if we force the lithographic process work with very small scales. This property is called as \textit{variability of lithographic process}. Hence, the connectivity of wires in devices can be converted as a random bit string which can be used as secret key (POK) in secure protocols. Moreover, this random string can be generated in reliable way. However, if the adversary can physically access the device to observe the connectivity of wires, then the security of this random string is not guaranteed anymore. As a second contribution, we propose a novel PCM-based POK. In the existing PCM-based PUFs~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, the resistances of two PCM cells, which are randomly defined by the process variation, are compared to produce a output bit. Due to the fluctuation in the current, the resistances can be changed and thus, the output is not reliable. Our proposed PCM-based POK is different from that in~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014} in terms of architecture, i.e., we use only one PCM cell to produce one bit output based on \textbf{the variability of granularity of PCM cells}. Thus, we can achieve a reliable PCM-based POK without using any reliability-enhancement techniques as mentioned above. Compared to the method based on lithographic process, since no-one can physically observe the granularity inside the PCM cell, the proposed PCM-based POK is secure against physical attacks. 
%
%The rest of the paper is organized as follows. We discuss related work in Section~\ref{sec:notation_background}. Section~\ref{sec:conclusion} concludes this paper. 

==> sections/related_works_old.tex <==
\section{Background and Related Work}
\label{sec:notation_background}

In this section, we provide a background and related works, i.e., reliability enhancement techniques, lithography based PUFs and PCM-based PUFs. 

\subsection{Reliability enhancement techniques}
\label{subsec:relibility_enhancement}

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{./figs/RepFE.pdf}
\caption{Reproduction Procedure of Fuzzy Extractors~\cite{dodis2004fuzzy}}
\label{fig:RepFE}
\end{figure}  


In the PUF's literature, to generate a random secret key which can be used in secure systems from the noisy source, two following problems must be solved: 1) Reliability and 2) de-correlation of raw output bits. 

\textbf{Reliability.} Since the raw output from noisy source is intrinsically noisy, we develop some approaches to produce a reliable raw output. Without loss of generality, we consider a POK with only single pair of challenge and response $\vect{(c,r)}$. Typically, there are two approaches to make the $\vect{r}$ reliable: \textbf{response reinforcement} and \textbf{ECC-based approach}

\textit{Reinforcement approach.} \ha{Nafisa's writing. The bad things for this approaches is: additional process, manpower and technique efforts required, and not general, i.e., only applied to bi-stable memory based POKs} 


\textit{ECC-based approach.} Compared to response reinforcement, this approach does not change the behavior of output permanently after doing additional process. Instead, an extra circuit which implements the error correction algorithm is required and we have the several constructions, e.g., Fuzzy Extractors (FEs)~\cite{dodis2004fuzzy}, Computational Fuzzy Extractors~\cite{FullerMengReyzin2013}, LPN-based PUFs~\cite{HerderRenDijkEtAl2016}. Without loss of generality, we focus on FE~\cite{dodis2004fuzzy}. A FE contains two procedures: $\mathrm{Gen}$ and $\mathrm{Rep}$. $\mathrm{Gen}$ takes the noisy output $W$ and true random string $s$ as the input and produces the output as $(h,s,k)$ where $h$ is the called helper data and $k$ is the secret key which is reliable and all its bits are independent. Helper data $h$ is used to reconstruct $W$ from its noisy version $W'$ generated from noisy source in Rep procedure by using an algorithm \textit{Secure Sketch} (SS) with a random bit input $x$, i.e., $h\leftarrow \mathrm{SS}(W,x)$. To generate $k$, a process is called \textit{Privacy Amplification} ($\mathrm{PA}$) is required, i.e.,  $k \leftarrow \mathrm{PA}(W,s)$. As shown in~\cite{dodis2004fuzzy}, the hash function is involved in PA. In a nutshell, $(h,s,k)\leftarrow \mathrm{Gen}(s,W)$. 

In Reproduction procedure (Rep), the raw POK output $W'$ is measured and it is a noisy version of $W$, i.e., $W'$ and $W$ are different in maximum $d$ positions or $d_{\mathrm{H}}(W',W)\leq d$. Typically, the helper data $h$ in Gen procedure is generated in a way such that the secure sketch SS can reconstruct $W$ from $W'$ with the condition $d_{\mathrm{H}}(W',W)\leq d$. Thus, $W \leftarrow \mathrm{SS}(W',h)$ and then the secret key $k$ is reproduced as $k \leftarrow \mathrm{PA}(W,s)$. Figure~\ref{fig:RepFE} depicts the Rep produce of FEs in~\cite{dodis2004fuzzy}. Compared to FEs, two constructions in~\cite{FullerMengReyzin2013,HerderRenDijkEtAl2016} also have two Gen and Rep, but they can correct more number of errors if the measurement noise in raw output follows \textit{independent and identically distributions} (i.i.d). Moreover, we can have many different types of ECC-based as shown in~\cite{Delvaux2014,Nguyen2015}. 

However, all the ECC-based approaches have the following problems.

\begin{itemize}
\item \textit{Security.} In FE construction~\cite{dodis2004fuzzy}, the security of $k$ is provided if the \textit{min-entropy} of raw output $W$ is known. However, this is \textit{impossible} mission in practice due to the large number of POK's output bits and all the bits are correlated. In other words, we cannot exactly address the security of POK-based system in the context of FEs. Moreover, the if the noise is big enough to make the condition $d_{\mathrm{H}}(W',W)\leq d$ does not hold, then security of FEs is also not guaranteed. In~\cite{FullerMengReyzin2013,HerderRenDijkEtAl2016}, since the two constructions are based on Learning Parity with Noise (LPN), the security is only provided when the measurement noise is \textit{i.i.d} which does not hold in practice. Moreover, we also need to know at least \textit{min-entropy} of $W$ for measuring the security of $k$ and thus, they also face the same problem for FE. More important, in~\cite{Delvaux2014,Nguyen2015}, it is shown that the existence of helper data $h$ can leak the information of the secret key $k$/ the raw output of POK $W$ or the adversary can fully retrieve the secret key/ the raw output $W$. 

\item \textit{Hardware Overhead.} As described in~\cite{dodis2004fuzzy,FullerMengReyzin2013,HerderRenDijkEtAl2016,Delvaux2014,Nguyen2015}, all ECC-based constructions require additional hardware circuitry such as True Random Number Generation, Error Correction Code algorithm (in Secure Sketch), Hash Functions (in Privacy Amplification), etc. Thus, beside the POK circuit, we need to implement several additional digital circuitry which makes the final hardware overhead is big. 

\item \textit{Efficiency.} Since many digital processes are involved in producing a secret key $k$, the efficiency of POK-based system significantly reduces in terms of execution time, power consumption. In~\cite{BhargavaCakirMai2012,BhargavaMai2013}, it is pointed that most ECC implementations $>2000$ cycles and $>3000$ SRAM bits to generate reliable 128-bit key $k$. 

\end{itemize}

From this analysis, we can see that all the problems mentioned above will be dropped if the raw outputs of POK is intrinsically reliable. Typically, \textit{response reinforcement} approach can solve all these problems but the shortcomings are: not general (i.e., only applied for bi-stable memory), manpower and technique efforts are in need and additional process is required.

\textbf{De-correlation.} As discussed above, all the raw output bits of POK (i.e., digital interpretation of analog output of POK) are correlated. Thus, we cannot directly use the raw output of POK as a secret key in secure systems. We need to de-correlate the raw output of POK by the privacy amplification process as described in ECC-based approaches if the raw output of POK is noisy. It is evident that, if PA is required, then the hardware overhead of system is increased and the efficiency of system is reduced.   

If the raw output is reliable (for example, after the response reinforcement), we can use a very simple trick in True Random Number construction, i.e., xoring several correlated bits together to produce a constructed bit. All constructed bits will be indepedent and identically distributed.  

\ha{Prof Marten: Why in FEs, we need PA instead of XOR trick? The input $W$ is reliable, and we can apply the XOR trick to the $W$. I am confused now at this point. It seems that something goes wrong here?????}

 
%To apply the output generated from a noisy random resource (for example POKs or PUFs) in secure systems, many types of error correction codes (ECCs) are proposed. Typically, the reliable and random bit string are required in secure systems and to do it, an extra information is produced based on the original output (a.k.a golden response) and it is called as \textit{helper data}. For the reproduction process, the output is measured again and it is usually noisy (i.e., has some mismatches with the golden response). This noisy output is combined with helper data to reconstruct the golden response by apply some ECC algorithms~\cite{Delvaux2014,Nguyen2015}. Actually, the existence of the helper data does not guarantee that the reproduction can be successfully done. All ECCs has a threshold for the number of errors presenting in noisy output. Moreover, the existence of helper data also hurts the security, hardware overhead and efficiency of the systems~\cite{Delvaux2014,Nguyen2015}. 
%
%Moreover, using ECCs only helps us to solve the reliability question, not the de-correlation problem if the noisy outputs are correlated. Thus, as shown in~\cite{dodis2004fuzzy}, the privacy amplification process is in need. Typically, the noisy output is collaborated with a short true random bit string (generated from a True Random Number Generator) and they are the input of a hash function. The output of hash function is provably random, i.e., not correlated or \textit{i.i.d.}. It is evident that this process significantly increases the hardware overhead reduces the efficiency of the system. 









\subsection{Lithography based PUFs}

%\cite{SreedharKundu2011,KumarBurleson2013,KumarDhanuskodiKundu2014} Lithograpy based PUFs

In optical lithography, devices and metal layers are printed in patterns on semiconductor wafers using a monochromatic light source which is focused through a lens system on a mask1. The entire IC fabrication process consists of several patterning, deposition, etching, doping, and polishing steps that comprise inherent variabilities and hence, prohibit precisely accurate reprint~\cite{Mack2007,KunduSreedharSanyal2007,KumarDhanuskodiKundu2014,SreedharKundu2011}. These variations in physical and electrical properties of the fabricated devices arise due to the aberrations in etching, doping and polishing steps, light source intensity imperfections, lens system and mask alignment issues, defocus, and interference problems~\cite{KumarDhanuskodiKundu2014}. 
Based on the everlasting consumer demands for smaller, faster, cheaper, and less energy hungry electronic devices, the expedition of the microelectronics industry has involved downsizing of the device feature size following Moore's Law for four decades~\cite{Moore1965}. However, the lack of improvements in the wavelength of the light source for past two decades led to the sub-wavelength lithographic approach where a larger wavelength of the light source (193 nm) is used for printing much narrower devices~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}. Due to the proximity effects, constructive or destructive interference from the slits of the mask result in wider or narrower printed lines~\cite{SreedharKundu2011}. The width variations can be significant enough to turn out zero line width or an open device in some of the destructive interference incidences with closely spaced pitches (defined as forbidden pitches)~\cite{KunduSreedharSanyal2007,KumarDhanuskodiKundu2014}. 
Even though several resolution enhancement techniques (such as optical proximity correction (OPC), alternating phase shift mask, and immersion lithography) are used to overcome these sub-wavelength lithographic challenges~\cite{KunduSreedharSanyal2007}, intentional avoidance of these schemes are also found in literature to engineer highly sensitive lithographic variations based PUFs (litho-PUFs)~\cite{KumarDhanuskodiKundu2014,SreedharKundu2011}. Exploiting linewidth, length, and height variations in lithography simulation of litho-PUFs with forbidden pitch, Sreedhar et al. demonstrated output voltage fluctuations as a function of focus variation in the simulated devices~\cite{SreedharKundu2011}. Kumar et al. addressed fluctuations in the light intensity and durations and focus variations due to wafer tilt and resist thickness variations and showed improved inter-die and inter-wafer uniqueness with lithography simulation in the forbidden pitch zone~\cite{KumarDhanuskodiKundu2014}.
Two types of variations are observed in the device properties, random and systematic. For improving the performance of litho-PUFs, the systematic variations are suppressed while keeping the random variations unaffected~\cite{KumarDhanuskodiKundu2014}. Forte et al. delineated OPC optimized for litho-PUF which enhances the random variations while reducing the systemic variations~\cite{Forte2012a,Forte2012}










%\subsection{Introduction of PCMs}
%
%To construct the Phase Change Memory storing the digital information, two different electrical resistivity of two alternative structural phases of a suitable material are exploited~\cite{ZhangKongChangEtAl2014}. Typically, PCM cell consists of a storage device and access device. The storage device is made in the way such that it can be programmed to either a low-resistivity \textit{crystalline phase} ($R \approx 10^2 \Omega$) or high-resistivity \textit{amorphous phase} ($R \approx 10^6 \Omega$) to represent the SET (logic-1) and the RESET (logic-0) state, respectively (see~\cite[Fig. 2]{ZhangKongChangEtAl2014}). To change the state from SET to RESET, a high magnitude and fast fall time pulse is applied to the storage device. Conversely, to change from RESET to the SET state, either a pulse with moderate magnitude and long duration is required. 

\subsection{PCM-based PUFs}

%In~\cite{ZhangKongChang2013,ZhangKongChangEtAl2014}, Zhang \textit{et.al} described proposed a PUF design based on PCM. At the same setup condition, the resistance of each PCM is randomly defined due to the process variation. Hence, by comparing the resistances of two different PCM cells, one random bit can be produced. However, if the environmental conditions change, then the resistance of PCM cell also changes. Thus, the proposed PCM-based PUF is not reliable.

Phase change memory (PCM) is an emerging non-volatile computer memory technology. It offers high speed, high endurance, low power programming and good cell scalability. A typical PCM cell consists of a phase change material (typically $Ge_2Sb_2Te_5$ or GST) between two electrodes. A portion of this material changes back and forth to high (amorphous, Rhigh) and low (crystalline, Rlow) resistance states when different electrical pulses are applied across the electrodes. The reversible transitions between these two states are called set (Rhigh to Rlow) and reset (Rlow to Rhigh). The read operation is performed with a small voltage by not disturbing the state of the cell~\cite{WongRaouxKimEtAl2010,burr2010phase}. 
The process variations and programming sensitivity of PCM is utilized in reconfigurable PUF implementation by Zhang et al. where dynamically updatable cryptographic keys are generated. The address of two selected PCM cells is used as the challenge and the resistance comparison of the two cells is the response~\cite{ZhangKongChangEtAl2014}. 




%\subsection{Resistance drift and decay of PCMs}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/resistance_drift.png}
%\caption{Resistance Drift and Decay of PCMs.}
%\label{fig:Drift_Decay_PCM}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width = \columnwidth]{./figs/resistance_drift_00.png}
%\caption{Resistance Drift and Decay of PCMs with different initial condition of RESET.}
%\label{fig:Drift_Decay_PCM_00}
%\end{figure}
%
%In order to build TLP based on PCM, the basic phenomena of PCM is exploited, i.e., the phenomena \textit{resistance drift and decay of PCM} as depicted in ~\cref{fig:Drift_Decay_PCM}. After the RESET with a certain initial condition (i.e., voltage and temparature), the resistance of PCM cell increases in the duration $[t_0,t_1]$ (the drift phase) and then it decreases after the saturation point $t_1$ (the decay phase). In~\cref{fig:Drift_Decay_PCM_00}, it is evident that the \textit{drift and decay} curve heavily depends on the initial condition of the RESET. Moreover, even if all the PCM cells are initialized under the same condition of the RESET, they have different curves of drift and decay. 



